Efficient Algorithms for Approximate Single-Source Personalized PageRank Queries

Given a graph $G$, a source node $s$ and a target node $t$, the personalized PageRank (PPR) of $t$ with respect to $s$ is the probability that a random walk starting from $s$ terminates at $t$. An important variant of the PPR query is single-source PPR (SSPPR), which enumerates all nodes in $G$, and returns the top-$k$ nodes with the highest PPR values with respect to a given source $s$. PPR in general and SSPPR in particular have important applications in web search and social networks, e.g., in Twitter's Who-To-Follow recommendation service. However, PPR computation is known to be expensive on large graphs, and resistant to indexing. Consequently, previous solutions either use heuristics, which do not guarantee result quality, or rely on the strong computing power of modern data centers, which is costly. Motivated by this, we propose effective index-free and index-based algorithms for approximate PPR processing, with rigorous guarantees on result quality. We first present FORA, an approximate SSPPR solution that combines two existing methods Forward Push (which is fast but does not guarantee quality) and Monte Carlo Random Walk (accurate but slow) in a simple and yet non-trivial way, leading to both high accuracy and efficiency. Further, FORA includes a simple and effective indexing scheme, as well as a module for top-$k$ selection with high pruning power. Extensive experiments demonstrate that the proposed solutions are orders of magnitude more efficient than their respective competitors. Notably, on a billion-edge Twitter dataset, FORA answers a top-500 approximate SSPPR query within 1 second, using a single commodity server.

==> 0-abstract/Abstract.tex <==
%!TEX root=../../ssppr.tex
\begin{abstract}
AA
\end{abstract} 

==> 0-commands/commands.tex <==

%\newtheorem{definition} {Definition}
%\newtheorem{example} {Example}
%\newtheorem{theorem} {Theorem}
%\newtheorem{lemma} {Lemma}
%\newtheorem{corollary} {Corollary}
%\newtheorem{problem} {Problem}
%\newtheorem{proposition} {Proposition}
%\newtheorem{assumption} {Assumption}
%\newtheorem{property} {Property}


\def\done{\hspace*{\fill} {$\square$}}
\def\header{\vspace{2.5mm} \noindent}
\def\extraspacing{\vspace{2mm}}
\def\myspacing{\vspace{2mm}}
\def\figcapup{\vspace{-2mm}}
\def\figcapdown{\vspace{-3mm}}
\def\tblcapup{\vspace{-0mm}}
\def\tblcapdown{\vspace{2mm}}
\def\tbldown{\vspace{-2mm}}
\def\tblup{\vspace{2mm}}
\def\codecapup{\vspace{-3mm}}
\def\codecapdown{\vspace{-2mm}}
\newcommand{\E}{{\mathbb E}}

\def\inN{N^{in}}
\def\outN{N^{out}}

\newcommand{\pf}{p_f}
\def\a{\alpha}
\def\dis{\sigma}
\def\err{\delta}
\def\eps{\epsilon}
\def\epi{\hat{\pi}}
\newcommand{\vect}[1]{\boldsymbol{#1}}
\def\rese{\pi^\circ}
\def\resi{r}
\def\rs{\pi^*}
\def\rd{r^*}

\def\rmax{r_{max}}

\def\ssppr{FORA}
\def\rsum{r_{sum}}

\def\correspondingauthor{\footnote{Corresponding author.}}


==> 2-Preliminaries/related__David_Yang_________________2017-02-18_.tex <==
%!TEX root=../ssppr_kdd17_newformat.tex

\section{Other Related Work} \label{sec:other-related}
%Existing solutions for personalized PageRank can be roughly divided into three categories: the matrix-based approaches \cite{JehW03,FujiwaraNYSO12,maehara2014computing,ZhuFCY13,berkhin2006bookmark,Chakrabarti07}, the local-update based approaches \cite{JehW03}, and the Monte-Carlo based approaches \cite{fogaras2005towards,BahmaniCX11,SarmaMPU13,lofgren2014fast,lofgren2015personalized,WangTXYL16}.


%
%PageRank and Personalized PageRank are first introduced by Page et al.\ \cite{page1999pagerank}. The former measures the global importance of a node in the graph, and the latter measures the importance of a node with respect to another node. Both problems have been extensively studied. We focus on the Personalized PageRank, and refer readers to \cite{Berkhin05} for detailed surveys on PageRank.
%
%In \cite{page1999pagerank}, Page et al.\ propose the {\em power iterations} approach to calculate the exact PPR vector with respect to a source node $s$ using Equation \ref{eqn:invariant}, where the PPR vector includes the PPR values for all $v \in V$ with respect to $s$. As explained in Section \ref{sec:existing-work}, this methods involves matrix operations on the adjacency matrix, which incurs high space and time costs for large graphs. Subsequently, a branch of research work focuses on developing algorithms to efficiently compute PPR vectors \cite{JehW03,FujiwaraNYSO12,maehara2014computing,ZhuFCY13,berkhin2006bookmark,fogaras2005towards,Chakrabarti07}. Jeh et al.\ \cite{JehW03} propose the backward search solution as discussed in Section \ref{sec:existing-work}, which is further optimized in \cite{fogaras2005towards,AndersenCL06}. Berkhin \cite{berkhin2006bookmark}, Chakrabarti \cite{Chakrabarti07}, and Zhu et al.\ \cite{ZhuFCY13} propose to (i) pre-compte the PPR vectors for some selected hub nodes, and then (ii) use the pre-computed results to answer PPR queries. However, Berkhin's method is limited to the case when the source is a distribution where all non-hub nodes have zero probabilities; Chakrabarti's and Zhu et al.'s techniques are based on variants of power iterations \cite{page1999pagerank} for PPR computation, and, thus, inherit its inefficiency for large graphs. Fujiwara et al.\ \cite{FujiwaraNYSO12} propose to pre-compute a QR decomposition of the adjacency matrix $A$ (see Section~\ref{sec:prelim}), and then utilize the results to accelerate PPR queries; nonetheless, the method incurs prohibitive preprocessing costs on million-node graphs. Later, Maehara et al. \cite{maehara2014computing} present a method that (i) decomposes the input graph into a core part and several tree-like structures, and then (ii) exploits the decomposition to speed up the computation of exact PPR vectors. Shin et al.\ \cite{ShinJSK15} propose {\em BEAR} to reorder the adjacency matrix of the input graph $G$ to obtain several easy-to-invert sparse sub-matrices. The sub-matrices are then stored as the index, and used to improve PPR query processing. This approach incurs prohibitive space consumption, and they further propose {\em BEAR-Approx} to reduce the index size by dropping values that are less than a dropout threshold $\gamma$ in the sub-matrices and setting them to zero. Nevertheless, as will be shown in our experiment, {\em BEAR-Approx} still incurs prohibitive preprocessing costs, and is not scalable to large graphs.
%
%
%In addition, the random walk based definition of PPR inspires a line of research work \cite{fogaras2005towards,BahmaniCX11,SarmaMPU13,lofgren2014fast,lofgren2015personalized} that utilizes the Monte-Carlo approach to derive approximate PPR results. In particular, Bahmani et al.\ \cite{BackstromL11} and Sarma et al.\ \cite{SarmaMPU13} investigate the acceleration of the Monte-Carlo approach in distributed environments. Fogaras et al.\ \cite{fogaras2005towards} presents a technique that pre-computes {\em compressed} random walks for PPR query processing, but the large space consumption of the technique renders it applicable only on small graphs. Lofgren et al.\ propose {\em FastPPR} \cite{lofgren2014fast}, which significantly outperforms the Monte-Carlo method in terms of query time. {\em FastPPR}, in turn, is subsumed by {\em BiPPR} \cite{lofgren2015personalized} in terms of query efficiency.
%
%There also exists a line of research work \cite{lofgren2015personalized,GuptaPC08,AvrachenkovLNSS11,BahmaniCX11,FujiwaraNYSO12,FujiwaraNSMO13sigmod} that investigates top-$k$ PPR queries. Nevertheless, almost all existing methods require that the target set $T=V$, i.e., the set of all nodes in the input graph. The only algorithm that supports arbitrary $T$ is {\em BiPPR}. In the next section, we show that {\em HubPPR} significantly outperforms {\em BiPPR} through extensive experimental results.


%\subsection{Existing Approximate Algorithms}\label{sec:related}

%\header
%{\bf Power-Iteration.} The {\em Power-Iteration} approach is first proposed by Page et al.\ \cite{page1999pagerank}. This approach is based on a recursive definition of PPR based on the following equation.
%\begin{equation}\label{eqn:powerit}
%\vect{\pi_s} = \a \cdot \vect{e_s} + (1-\a)\cdot \vect{\pi_s}\cdot D^{-1}A.
%\end{equation}
%where $A \in \{0, 1\}^{n\times n}$ is the adjacency matrix of $G$, and  $D\in R^{ n \times n}$ is a diagonal matrix  in which each element on its main diagonal corresponds to a node $v$, and its value is the out degree of $v$. The {\em Power-Iteration} approach first makes an initial guess of $\vect{\pi_s}$, e.g., $(\frac{1}{n}, \cdots, \frac{1}{n})$. Afterwards, it repeatedly applies the current $\vect{\pi_s}$ to the RHS of Equation \ref{eqn:powerit}, and derives the new solution of $\vect{\pi_s}$. As shown in \cite{haveliwala2003second}, to achieve an additive error of $\delta$ for each node $v$, i.e., $|\epi(s,v)- \pi(s,v)|\le \delta$ , $O\left(\log{\frac{1}{\delta}}\right)$ iterations are sufficient. However, the computation cost of each iteration is $O(m)$, and hence the total time complexity is $O\left(m\cdot \log{\frac{1}{\delta}}\right)$

%This section surveys the related work. Sections \ref{sec:related-mc} and \ref{sec:related-bi} review the methods most relevant to ours, while Section~\ref{sec:related-other} reviews the other techniques.

%\subsection{BiPPR Approach} \label{sec:related-bi}


%when a target set $T$ is given, and propose efficient algorithms for $|T|\le 10,000$. However, the proposed solutions do not work for the case when $V= T$. In \cite{WangTXYL16}, Wang et al. also propose efficient indexing scheme for the point-to-point PPR queries and the top-$k$ PPR queries with a target set $T$. However, the indexing approach cannot be directly applied to the single-source PPR queries and the top-$k$ PPR queries on the entire node set, hence we omit the results in \cite{WangTXYL16}.

%to out best knowledge, there still exist no efficient solutions for the top-$k$  PPR queries under the {\em BiPPR} framework when  $T=V$.

%Despite the fact that the cost of {\em BiPPR} is much lower than the {\em MC} approach for point-to-point PPR queries, its costs for the single-source and top-$k$ PPR queries are still very high as will be shown in our experiment in Section \ref{sec:exp}.

%In \cite{LofgrenBG15}, Peter et al. further propose the point-to-point PPR query with worst case time complexity of $O\left( \frac{1}{\eps}\sqrt{\frac{d_{max}\cdot \log{(1/\pf)}}{ \delta}}\right)$ on undirected graphs. The key observation is that on undirected graphs, $\pi(s,t) = |\outN(t)|\cdot \pi(t,s)/|\outN(s)|$. The idea is similar to {\em BiPPR} except that it does forward local update from the source $s$, and does random walks from the target node $t$. However, the proposed approach is restricted on undirected graphs, while in most real applications, the underlying graphs are directed.

%With this property and Equation \ref{eqn:bippr}, Peter et al.\ \cite{lofgren2015personalized} proves that the total number of required random walks can be reduced to $O\left(\rmax\cdot\frac{\log{((1/\pf))}}{\eps^2 \delta}\right)$.
%With Equation \ref{eqn:bippr},
%By setting $\rmax$ to $O\left(\eps\cdot\sqrt{\frac{m\cdot \delta}{n\cdot\log{(1/\pf)}}}\right)$, they show that the amortized cost of the  {\em BiPPR}  is $O\left( \frac{1}{\eps}\sqrt{\frac{m\cdot \log{(1/\pf)}}{n\cdot \delta}}\right)$ for point-to-point PPR queries.

%This approach can be also applied to the single source PPR queries by conducting $n$ point-to-point PPR queries from $s$ to each node $v\in V$.
%The high level idea of the {\em BiPPR} is that it conducts a forward phase from the source node $s$ and a backward phase from the target node $t$. The forward phase is similar to that of the {\em MC} approach, by simulating random walks from $s$. The backward phase calculates an estimated PPR $\epi(v,t)$ for the target node $t$ with respect to each node $v\in V$. In particular, the backward phase propagates an unit message from $t$, and examine how much is propagated to each node. For each node $v$, the backward phase maintains a reserve $\rese(v,t)$ to denote the estimated PPR for $\pi(v,t)$, and  a residue $\resi(v,t)$ to indicate the amount of message that will be propagated by node $v$. Initially, the residue and reserve of all nodes are set to zero except the residue of target t, which is set to 1. Afterwards, it entails a backward push operation from a node $v$ that: {\em (i)} adds $\a$ portion of its current residue, i.e., $\a\cdot \resi(v,t)$,  to its reserve; {\em (ii)} adds $(1-\a)\cdot \resi(v,t)\cdot \frac{|\outN(u)|}{|\inN(v)|}$ to the residue of each  $u\in \inN(v)$, where $\inN(u)$ (resp.\ $\outN(u)$) denotes the in-neighbors (resp.\ out-neighbors) of node $u$; {\em (iii)} set $\resi(v,t)$ to zero. The backward phase terminates when the residue of any node is smaller than $\rmax$, a predefined threshold for backward phase.
%It is proven in \cite{AndersenBCHMT07} that, the following invariant holds:
%\begin{equation}\label{eqn:bippr}
%\pi(s,t) = \rese(s,t) + \sum_{v\in V} r(v,t) \cdot \pi(s,v).
%\end{equation}
%It has been proved in \cite{AndersenBCHMT07} that, the reserve and residue satisfies the following Equation:
%\begin{equation}
%\pi(s,t) = \rese(s,t) + \sum_{v\in V} \resi(v,t)\cdot \pi(s,v)
%\end{equation}
%Peter et al. further proves that the amortized cost for the backward phase is $O\left(\frac{m}{n\cdot \rmax}\right)$. Note that when the backward propagation terminates, $\resi(v,t)< \rmax$ for all nodes.
%%and the number of random walks can be reduced to $O\left( \frac{3\cdot \rmax \cdot \log{(1/\pf)}}{\eps^2 \delta}\right)$ to satisfy Equation \ref{eqn:ss-def} for target $t$ with $1-\pf$ probability.
%%As $r(v,t)< \rmax$, by setting $\sum_{v\in V} r(v,t) \cdot \pi(s,v)$
%With this property and Equation \ref{eqn:bippr}, Peter et al.\ \cite{lofgren2015personalized} proves that the total number of required random walks can be reduced to $O\left(\rmax\cdot\frac{\log{((1/\pf))}}{\eps^2 \delta}\right)$.
%%With Equation \ref{eqn:bippr},
%By setting $\rmax$ to $O\left(\eps\cdot\sqrt{\frac{m\cdot \delta}{n\cdot\log{(1/\pf)}}}\right)$, they show that the amortized cost of the  {\em BiPPR}  is $O\left( \frac{1}{\eps}\sqrt{\frac{m\cdot \log{(1/\pf)}}{n\cdot \delta}}\right)$ for point-to-point PPR queries.
%
%This approach can be also applied to the single source PPR queries by conducting $n$ point-to-point PPR queries from $s$ to each node $v\in V$.


%For single-source PPR queries, we note that {\em BiPPR} could actually achieve the same time complexity as {\em \ssppr}.
%than simply doing $n$ point-to-point PPR queries with $\rmax =O\left(\eps\cdot\sqrt{\frac{m\cdot \delta}{n\cdot\log{1/\pf}}}\right)$, in which case the time complexity is $O\left( \frac{n}{\eps}\sqrt{\frac{m\cdot \log{1/\pf}}{n\cdot \delta}}\right)$.
%In particular, notice that the amortized cost to do the backward phase is $O\left(\frac{m}{n\cdot \rmax}\right)$. Hence, if $n$ nodes do the backward phase with the same $\rmax$, the total cost is $O\left(\frac{m}{\rmax}\right)$. The time complexity of {\em BiPPR} for single-source PPR query hence is $O\left(\frac{m}{\rmax}+\rmax\cdot\frac{\log{(1/\pf)}}{\eps^2 \delta}\right)$. By setting $\rmax=O\left(\eps\cdot\sqrt{\frac{m\cdot \delta}{\log{(1/\pf)}}}\right)$, it derives the same time complexity as {\em \ssppr}. Nevertheless, as will be shown in our experiment, the proposed {\em \ssppr} is generally several times faster than {\em BiPPR}, and can be orders of magnitude faster than {\em BiPPR} by leveraging our proposed light-weighted index.
%
%In \cite{lofgren2015personalized, WangTXYL16}, they study the top-$k$ PPR queries under the {\em BiPPR} framework when a target set $T$ is given, and propose efficient algorithms for $|T|\le 10,000$. However, the proposed solutions do not work for the case when $V= T$. In \cite{WangTXYL16}, Wang et al. also propose efficient indexing scheme for the point-to-point PPR queries and the top-$k$ PPR queries with a target set $T$. However, the indexing approach cannot be directly applied to the single-source PPR queries and the top-$k$ PPR queries on the entire node set, hence we omit the results in \cite{WangTXYL16}.
%
%%to out best knowledge, there still exist no efficient solutions for the top-$k$  PPR queries under the {\em BiPPR} framework when  $T=V$.
%
%%Despite the fact that the cost of {\em BiPPR} is much lower than the {\em MC} approach for point-to-point PPR queries, its costs for the single-source and top-$k$ PPR queries are still very high as will be shown in our experiment in Section \ref{sec:exp}.
%
%In \cite{LofgrenBG15}, Peter et al. further propose the point-to-point PPR query with worst case time complexity of $O\left( \frac{1}{\eps}\sqrt{\frac{d_{max}\cdot \log{(1/\pf)}}{ \delta}}\right)$ on undirected graphs. The key observation is that on undirected graphs, $\pi(s,t) = |\outN(t)|\cdot \pi(t,s)/|\outN(s)|$. The idea is similar to {\em BiPPR} except that it does forward local update from the source $s$, and does random walks from the target node $t$. However, the proposed approach is restricted on undirected graphs, while in most real applications, the underlying graphs are directed.


%In \cite{lofgren2015personalized, WangTXYL16}, they study the top-$k$ PPR queries under the {\em BiPPR} framework when a target set $T$ is given, and propose efficient algorithms for $|T|\le 10,000$. However, to out best knowledge, there still exist no efficient solutions for the top-$k$  PPR queries under the {\em BiPPR} framework when  $T=V$.


%\subsection{Other Methods} \label{sec:related-other}
An important category of existing solutions for personalized PageRank is the {\em matrix-based} approaches \cite{JehW03,FujiwaraNYSO12,maehara2014computing,ZhuFCY13,berkhin2006bookmark,Chakrabarti07,JehW03,ZhangLG16,AndersenBCHMT07,AndersenCL06,ZhangLG16}. Let $\vect{\pi_s}$ be the PPR vector for source $s$. The matrix-based approaches  target to solve the following equation:
\begin{equation}\label{eqn:powerit}
\vect{\pi_s} = \a \cdot \vect{e_s} + (1-\a)\cdot \vect{\pi_s}\cdot D^{-1}A.
\end{equation}
where $A \in \{0, 1\}^{n\times n}$ is the adjacency matrix of $G$, and  $D\in R^{ n \times n}$ is a diagonal matrix  in which each element on its main diagonal corresponds to a node $v$, and its value is the out degree of $v$.

The first matrix-based solution for the single PPR query is the {\em Power-Iteration} approach, proposed by Page et al. \cite{page1999pagerank}. It first makes an initial guess of $\vect{\pi_s}$, e.g., $(\frac{1}{n}, \cdots, \frac{1}{n})$, and then repeatedly applies the current $\vect{\pi_s}$ to the RHS of Equation \ref{eqn:powerit}, and derives the new solution of $\vect{\pi_s}$. It terminates when all elements converge. However, the {\em Power-Iteration} approach requires $\Omega(m)$ time to answer a query, which is too slow for large graphs, and a line of research work focused on improving the efficiency of the single PPR queries\cite{FujiwaraNYSO12,maehara2014computing,ZhuFCY13}. Fujiwara et al.\ \cite{FujiwaraNYSO12}, Maehara et al.\ \cite{maehara2014computing}, and Shin et al.\ \cite{ShinJSK15} propose to decomposes the input graph into tree structures or sub-matrices, and use them to speedup the query.  The state-of-the-art approach for the single-source and top-$k$ PPR queries in this line of research work is {\em BEAR} proposed by Shin et al.\ \cite{ShinJSK15}. In particular, they propose to reorder the adjacency matrix of the input graph $G$ to obtain several easy-to-invert sparse sub-matrices. The sub-matrices are then stored as the index, and used to improve PPR query processing. However, this approach is subsumed by {\em HubPPR} \cite{WangTXYL16} in terms of query efficiency and accuracy.


Another category of existing solutions is the {\em local update} approaches. This approach is a local version of the {\em Power-Iteration} approach, which avoids the significant cost of maintaining the matrices in the matrix-based approaches. Andersen et al.\ \cite{AndersenCL06} propose the forward push algorithm as described in Section \ref{sec:ss-lp}. Berkin et al.\ \cite{Berkhin05} further propose to pre-compute the forward push results from several important nodes, and then use these results to speedup the query performance.
Ohsaka et al.\ \cite{OhsakaMK15} and Zhang et al.\ \cite{ZhangLG16} further design algorithms to update the stored forward push results on dynamic graphs. However, none of existing solutions in this category provide approximation guarantee for single-source or top-$k$ PPR query algorithms on directed graphs.  Jeh et al.\ \cite{JehW03} propose the backward search solution, the reverse local variant of the forward push algorithm, which calculates the estimated PPRs from all nodes to a target node $t$. The backward search algorithm is further optimized in \cite{fogaras2005towards,AndersenCL06}. Zhang et al.\ \cite{ZhangLG16} also design the algorithms to update the stored backward push results on dynamic graphs. However, these approaches cannot support single-source PPR query or top-$k$ PPR queries.


Another category of existing solution is the random walk based approach. The aforementioned {\em MC} approach and {\em BiPPR} both fall into this category. Besides these two work, Fogaras et al.\ \cite{fogaras2005towards} propose techniques to pre-store the random walk results, and use them to speedup the query processing. However, the large space consumption of the technique renders it applicable only on small graphs. Bahmani et al.\ \cite{BackstromL11} and Sarma et al.\ \cite{SarmaMPU13} investigate the acceleration of the Monte-Carlo approach in distributed environments.  Lofgren et al.\ propose {\em FastPPR} \cite{lofgren2014fast}, which significantly outperforms the Monte-Carlo method in terms of query time. {\em FastPPR}, in turn, is subsumed by {\em BiPPR} \cite{lofgren2015personalized} in terms of query efficiency.

In \cite{lofgren2015personalized,GuptaPC08,AvrachenkovLNSS11,BahmaniCX11,FujiwaraNYSO12,FujiwaraNSMO13sigmod}, they also investigate the top-$k$ PPR queries. Gupta et al.\  \cite{GuptaPC08}  propose to use forward push to return the top-$k$ answers. However, their solutions do not provide any approximation guarantee. Avrachenkov et al.\ \cite{AvrachenkovLNSS11} study how to use Monte-Carlo approach to  find the top-$k$ nodes. However the solution does not return estimated PPR values and does not provide any approximation guarantee. Fujiwara et al.\ \cite{FujiwaraNYSO12,FujiwaraNSMO13sigmod} and Shin et al.\cite{ShinJSK15} study how to speedup the top-$k$ PPR queries with the matrix decomposition approach. These approaches either cannot scale to large graphs or do not provide approximation guarantees.
%Jeh et al.\ \cite{JehW03} propose the backward search solution, which is further optimized in \cite{fogaras2005towards,AndersenCL06}. Berkhin \cite{berkhin2006bookmark}, Chakrabarti \cite{Chakrabarti07}, and Zhu et al.\ \cite{ZhuFCY13} propose to (i) pre-compte the PPR vectors for some selected hub nodes, and then (ii) use the pre-computed results to answer PPR queries.  However, Berkhin's method is limited to the case when the source is a distribution where all non-hub nodes have zero probabilities; Chakrabarti's and Zhu et al.'s techniques are based on variants of power iterations \cite{page1999pagerank} for PPR computation, and, thus, inherit its inefficiency for large graphs.

%Fujiwara et al.\ \cite{FujiwaraNYSO12} propose to pre-compute a QR decomposition of the adjacency matrix $A$ (see Section~\ref{sec:prelim}), and then utilize the results to accelerate PPR queries; nonetheless, the method incurs prohibitive preprocessing costs on million-node graphs. Later, Maehara et al. \cite{maehara2014computing} present a method that (i) decomposes the input graph into a core part and several tree-like structures, and then (ii) exploits the decomposition to speed up the computation of exact PPR vectors.

%The state-of-the-art matrix-based approach is {\em BEAR} proposed by Shin et al.\ \cite{ShinJSK15}. In particular, they propose to reorder the adjacency matrix of the input graph $G$ to obtain several easy-to-invert sparse sub-matrices. The sub-matrices are then stored as the index, and used to improve PPR query processing. However, this approach does not provide any approximation guarantee for the queries, and cannot scale to large graphs as shown in \cite{WangTXYL16}.



%However, this approach incurs $O(n^2)$ space to store the adjacency matrix, and  and motivates a line of research work to further improve the query efficiency.

%As shown in \cite{haveliwala2003second}, to achieve an additive error of $\delta$ for each node $v$, i.e., $|\epi(s,v)- \pi(s,v)|\le \delta$ , $O\left(\log{\frac{1}{\delta}}\right)$ iterations are sufficient. However, the computation cost of each iteration is $O(m)$, and hence the total time complexity is $O\left(m\cdot \log{\frac{1}{\delta}}\right)$

%The first solution to calculate the single source PPR is the {\em power iterations} approach, proposed by Page et al. \cite{page1999pagerank}. The approach first makes an initial guess on the PPR scores with respect to the source $s$, and then iteratively refines the result


%Existing solutions for personalized PageRank can be roughly divided into two categories: the matrix-based approaches  and the Monte-Carlo based approaches \cite{fogaras2005towards,BahmaniCX11,SarmaMPU13,lofgren2014fast,lofgren2015personalized,WangTXYL16}.

%Among the matrix-based approaches, the first solution to calculate the single source PPR is the {\em power iterations} approach, proposed by Page et al. \cite{page1999pagerank}.

%In \cite{page1999pagerank}, Page et al.\ propose the {\em power iterations} approach to calculate the exact PPR vector with respect to a source node $s$ using Equation \ref{eqn:invariant}, where the PPR vector includes the PPR values for all $v \in V$ with respect to $s$. 

==> 6-Exp/exp__Fox_Mulder_s_conflicted_copy_2017-02-18_.tex <==
%!TEX root=../ssppr_kdd17_newformat.tex

\section{Experiments} \label{sec:exp}

In this section, we experimentally evaluate {\em \ssppr} and its index-based variant, referred to as {\em \ssppr+}, against the state of the art. All experiments are conducted on a Linux machine with an Intel 2.6GHz CPU and 64GB memory.

\begin{table}[t]
\centering
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|r|r|r|c|}
    \hline
    {\bf Name} & \multicolumn{1}{c|}{$\boldsymbol{n}$} & \multicolumn{1}{c|}{$\boldsymbol{m}$} & \multicolumn{1}{c|}{\bf Type}  & \multicolumn{1}{c|}{\bf Linking Site}\\
%    \hline
    \hline
    {\em DBLP}   &613.6K    & 2.0M          & undirected & www.dblp.com\\% 1 \\
    \hline
    {\em Web-St}      & 281.9K    & 2.3M      & directed & www.stanford.edu\\
    \hline
    {\em Pokec}      & 1.6M    &30.6M      & directed & pokec.azet.sk \\
    \hline
    {\em LJ} & 4.8M & 69.0M    & directed &  www.livejournal.com \\
    \hline
    {\em Orkut}      & 3.1M    & 117.2M      & undirected  & www.orkut.com \\
    \hline
    {\em Twitter}   & 41.7M & 1.5B & directed & twitter.com\\
    \hline
\end{tabular}
\vspace{1mm}
\caption{Datasets. ($K=10^3, M=10^6, B=10^9$)} \label{tbl:exp-data}
\end{small}
\vspace{-6mm}
\end{table}



\subsection{Experimental Settings}


%\header
{\bf Datasets and query sets.} We use 6 real graphs: {\em DBLP}, {\em Web-St}, {\em Pokec},  {\em LJ}, {\em Orkut}, and {\em Twitter}, which are benchmark datasets used in recent work \cite{lofgren2015personalized,WangTXYL16}. Table \ref{tbl:exp-data} summarizes the statistics of the data. For each dataset, we choose $50$ sources nodes uniformly at random, and we generate a single-source PPR query from each chosen node. In addition, we also generate $5$ top-$k$ queries from each source node, with $k$ varying in $\{100, 200, 300, 400, 500\}$. Note that the maximum $k$ is set to $500$ in accordance to Twitter's Who-To-Follow service \cite{gupta2013wtf}, whose first step requires deriving top-$500$ PPR results.

\header
{\bf Methods.} For whole-graph SSPPR queries, we compare our proposed {\em \ssppr} and {\em \ssppr+} against three methods: (i) the {\em Monte-Carlo} approach, dubbed as {\em MC}; (ii) the optimized {\em BiPPR} for SSPPR queries described in Appendix \ref{app:ssbippr}; (iii) {\em HubPPR}, which is the indexed version of {\em BiPPR}. For fair comparison, the index size of {\em HubPPR} is set to be the same as that of {\em \ssppr+}. For top-$k$ PPR queries, we compare our algorithm with single-source MC and single-source {\em BiPPR}, as well as the top-$k$ algorithm for {\em HubPPR} in \cite{WangTXYL16}. Following previous work\cite{lofgren2014fast,lofgren2015personalized,WangTXYL16}, we set $\delta = 1/n, \pf = 1/n$, and $\eps=0.5$. %For {\em HubPPR}, the index size is set to the same as {\em \ssppr+}.


\subsection{Whole-Graph SSPPR Queries} \label{sec:exp-ss}


In our first set of experiments, we evaluate the efficiency of each method for single-source PPR queries. Table \ref{tbl:ppr-query} reports the average query time of each method. Observe that both {\em \ssppr} and {\em BiPPR} achieve better query performance than {\em MC}, which is consistent with our analysis that the time complexity of {\em \ssppr} and {\em BiPPR} is better than that of {\em MC}. Moreover, {\em \ssppr} is at least $3$ times faster than {\em BiPPR} on most of the datasets. %For instance, on Twitter, {\em \ssppr} is around 3.7x faster than {\em BiPPR}.
The reason, as we explain in Section \ref{sec:ana}, is that {\em BiPPR} requires conducting a backward search from each node $v$ in $G$, even if $\pi(s, v)$ is extremely small. In contrast, {\em \ssppr} tends to omit nodes with small PPR values, which helps improve efficiency.

In addition, {\em \ssppr+} achieves significant speedup over {\em \ssppr}, and is around 10 times faster the latter on most of the datasets. %This is due to our advanced design of the index structure according to our theoretical analysis in Section \ref{sec:ana}.
The {\em HubPPR} also improves over {\em BiPPR}, but the improvement is far less than what {\em \ssppr+} achieves over {\em \ssppr}. %The reason is that, for single-source PPR queries, the number of required random walks is much larger than that in point-to-point PPR queries. Hence, when the stored random walks are consumed on a hub, and it needs to do random walks online.
Moreover, even without any index, {\em \ssppr} is still more efficient than {\em HubPPR}. %which indicates that the proposed {\em \ssppr} is more favorable choice on single-source PPR queries than other alternatives.


\begin{table}[!t]
\centering
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{center}
  \begin{tabular}{ | p{0.88cm} | r | r|r|r |r|}
    \hline
        & {\em MC} & {\em BiPPR} & {\em HubPPR}&   {\em \ssppr} & {\em \ssppr+}\\
    \hline
 {\em DBLP}  &12.9 &	3.2&  	1.7&	0.7	& 0.07   \\
    \hline
{\em Web-St}  & 5.0	&3.5&  	2.1	&0.03	&  0.01 \\
    \hline
 {\em Pokec} &66.4	&23.7& 17.3& 12.1	& 0.8 \\
    \hline
 {\em LJ}&144.7	& 46.7& 	30.1	& 21.0	&1.8  \\
    \hline
{\em Orkut} &241.4	& 156.2 &104.2	& 46.4	& 4.9	 \\
    \hline
{\em Twitter}   &4.6K	&3.3K& 	 2.6K & 891.5	&103.1 	\\
    \hline
  \end{tabular}
  \vspace{1mm}
  \caption{Single-source query performance (s). ($K=10^3$) } \label{tbl:ppr-query}
  \vspace{-6mm}
\end{center}
\end{small}
\end{table}


\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
%    \begin{footnotesize}
    \begin{tabular}{cccc}
      %\multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figs/topk_query_legend.eps}}  \\[-2mm]
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/dblp-topk-time.eps} &
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/pokec-topk-time.eps}&
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/orkut-topk-time.eps} &
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/tw-topk-time.eps}
   \\[-1mm]
        \hspace{-4mm} (a) DBLP  &
        \hspace{-4mm} (b) Pokec &
        \hspace{-4mm} (c) Orkut &
        \hspace{-4mm} (d) Twitter \\[-1mm]
 \end{tabular}
\vspace{-2mm}
 \caption{Top-$k$ PPR query efficiency: varying $k$.} \label{exp:topk-time}
\vspace{-0mm}
\end{figure*}
\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
%    \begin{footnotesize}
    \begin{tabular}{cccc}
      \multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figure/algo-legend.eps}}  \\[0mm]
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/dblp-topk-prec.eps} &
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/pokec-topk-prec.eps}&
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/lj-topk-prec.eps} &
        \hspace{-6mm} \includegraphics[height=32mm]{./figure/topk/orkut-topk-prec.eps}
   \\[-1mm]
        \hspace{-4mm} (a) DBLP  &
        \hspace{-4mm} (b) Pokec &
        \hspace{-4mm} (c) LJ &
        \hspace{-4mm} (d) Orkut \\[-1mm]
 \end{tabular}
\vspace{-2mm}
 \caption{Top-$k$ PPR query accuracy: varying $k$.} \label{exp:topk-acc}
\vspace{-0mm}
\end{figure*}

\subsection{Top-$\boldsymbol k$ SSPPR Queries} \label{sec:exp-topk}
%$This section evaluates the efficiency and accuracy of the proposed top-$k$ PPR query algorithms against the states-of-the-art.
%
In our second set of experiments, we evaluate the efficiency and accuracy of each method for top-$k$ PPR queries. Figures \ref{exp:topk-time} reports average the query time of each method on four representative datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, and {\em Twitter}. (The results on the other two datasets are qualitatively similar, and are omitted due to the space constraint.) Note that the y-axis is in log-scale. The main observation is that {\em \ssppr} and {\em \ssppr+} both considerably outperform competitors. In particular, {\em \ssppr} is up to two orders of magnitude faster than {\em MC} and {\em BiPPR}. This is expected since our top-$k$ algorithm applies an iterative approach to refine the top-$k$ answers and terminates immediately whenever the answer could provide the desired approximation guarantee. {\em HubPPR}'s top-$k$ algorithm has a similar early-termination mechanism, but it is outperformed even by the index-free {\em \ssppr}. The reason is that {\em HubPPR} requires performing a large number of backward searches, as is the case for {\em BiPPR}.
%
%%Nevertheless, even without index, our {\em \ssppr} is still several times faster than {\em HubPPR}. With full-fledged index, our {\em \ssppr+} is an order of magnitude faster than {\em HubPPR} approach.
%

To compare the accuracy of the top-$k$ results returned by each method, we first calculate the ground-truth answer of the top-$k$ queries using {\em MC} with $\eps = 0.01$, i.e., we perform $O(10000n\cdot \log n)$ random walks from each source node on each graph. Afterwards, we evaluate the top-$k$ results of each algorithm in terms of their precision with respect to the ground truth. Figure~\ref{exp:topk-acc} shows the accuracy of the top-$k$ query algorithms on four datasets: {\em DBLP}, {\em Pokec}, {\em LJ}, and {\em Orkut}. (We omit {\em Twitter} due to the prohibitive time required to compute the ground truth.) Observe that, {\em \ssppr}, {\em \ssppr+}, {\em BiPPR}, and {\em HubPPR} all achieve better accuracy than {\em MC}. %To explain, all these four algorithms include a local update algorithm, either forward push or backward push, and provides a deterministic part, i.e., $\rese(s,v)$, and then use random walks to approximate the remaining part. However, the {\em MC} approach only use the random walks to estimate the PPRs, which is less accurate than the other solutions.


\subsection{Preprocessing Costs}

Finally, we inspect the preprocessing costs of the two index-based methods, {\em \ssppr+} and {\em HubPPR}. As shown in Table \ref{tbl:exp-preprocessing}, the preprocessing time of {\em \ssppr} and {\em HubPPR} are both moderate, and the cost of {\em \ssppr} is much smaller than that of {\em HubPPR}. In addition, even on the largest dataset Twitter, {\em \ssppr+} can finish index construction in less than an hour. %This process can be further parallelized to reduce the preprocessing time.
Table \ref{tbl:exp-preprocessing} also reports the index size of {\em \ssppr+} and {\em HubPPR}. We also add the space consumption of the input graph as the reference values. As we can observe, the index size of {\em \ssppr+} is no more than 4 times the original graph in general. In particular, on {\em Orkut}, the index size of {\em \ssppr+} is only only 1.7 times the input graph, as yet, as we show in Sections \ref{sec:exp-ss} and \ref{sec:exp-topk}, it can speedup the query efficiency of single-source and top-$k$ PPR queries by around 10 times. This demonstrates the effectiveness and efficiency of our indexing scheme.
%, and that our index scheme is more favorable choice on single-source and top-$k$ PPR queries.





%
%\begin{table}[!t]
%\centering
%\begin{small}
%\renewcommand{\arraystretch}{1.1}
%\begin{center}
%\hspace*{-3mm}
%  \begin{tabular}{|p{1.2cm}|r| r | r|r|r|r|r|r|}
%    \hline
%      &{\bf Datasets} &  {\em DBLP}&   {\em Web-St} & {\em Pokec} & {\em LJ} &{\em Orkut} & {\em Twitter}\\
%       \hline
%     \multirow{2}{*}{\parbox{1.2cm}{Indexing time (s)}} &  {\em \ssppr+} &4.9	&2.0 & 38.6 & 97.1	& 204.9	& 3335.1 \\
%      \cline{2-8}
%      &  {\em HubPPR}  &28.7 	& 11.8 & 11.27 & 307.1	& 582.3	& 5846.1	\\
%        \hline
%         {\parbox{1.2cm}{Graph size}}&--- & 18.4MB & 10.4MB & 130.8MB & 295.2MB&950.1MB &6.16GB\\
%        \hline
%        {\parbox{1.2cm}{Index size}}&--- & 90.8MB & 45.5MB & 411.9MB & 1.1GB&1.6GB & 12.6GB\\
%        \hline
%%             \multirow{2}{*}{\parbox{1.2cm}{Index size (MB)}} &  {\em \ssppr+} &4.9	&2.0 & 38.6 & 97.1	& 204.9	& 3335.1 \\
%%      \cline{2-8}
%%      &  {\em HubPPR}  &28.7 	& 11.8 & 11.27 & 307.1	& 582\href{}{}.3	& 5846.1	\\
%%        \hline
%  \end{tabular}
%\caption{Preprocessing cost: {\ssppr+} v.s. {\em HubPPR}. } \label{tbl:ppr-preprocessing}
%\vspace{-2mm}
%\end{center}
%\end{small}
%\end{table}



\begin{table}[!t]
\vspace{-3mm}
\centering
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{center}
\hspace*{-3mm}
  \begin{tabular}{ | p{0.9cm} | r | r|r |r|}
    \hline
      \multirow{2}{*}{\bf Datasets}  & \multicolumn{2}{c|} {\bf Preprocessing time (sec)} &\multicolumn{2}{c|} {\bf Space consumption}  \\
    \cline{2-5}
     & {\em HubPPR} &  \multicolumn{1}{c|}{\em \ssppr+}  & { Index size} &   \multicolumn{1}{c|}{ Graph size} \\
    \hline
 {\em DBLP} & 28.7 &	 4.9&	90.8MB	& 18.4MB  \\
    \hline
{\em Web-St}  &  11.8 & 2.0& 45.5MB	& 10.4MB \\
    \hline
 {\em Pokec} &112.3 &	38.6&411.9MB	& 130.8MB \\
    \hline
 {\em LJ}& 307.9	&97.1 & 1.1GB	&295.2MB  \\
    \hline
{\em Orkut} &582.2	&204.9&1.6GB	& 950.1MB \\
    \hline
{\em Twitter}   &5849.0 &	3335.1& 12.6GB&6.2GB 	\\
    \hline
  \end{tabular}
\caption{Preprocessing costs. } \label{tbl:exp-preprocessing}
\vspace{-4mm}
\end{center}
\end{small}
\end{table}




==> 6-Exp/exp__Runhui_Wang_s_conflicted_copy_2019-03-14_.tex <==
%!TEX root=../ssppr_kdd17_newformat.tex

\section{Experiments} \label{sec:exp}

In this section, we experimentally evaluate our methods for whole-graph SSPPR queries and top-$k$ SSPPR queries. For whole-graph (resp. top-$k$) SSPPR queries, we include our index free methods {\em \ssppr}, which includes the optimizations as mentioned in Section \ref{sec:opt} (resp. Section \ref{sec:topk-running-time-guarantee}),  and their index-based variant, referred to as {\em \ssppr+}, against the states of the art. All experiments are conducted on a Linux machine with an Intel 2.9GHz CPU and 200GB memory.

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
%\tbl{Datasets. ($K=10^3, M=10^6, B=10^9$\label{tbl:exp-data})}{
\caption{Datasets. ($K=10^3, M=10^6, B=10^9$)}
\label{tbl:exp-data}
\begin{tabular}{|l|r|r|r|c|}
    \hline
    {\bf Name} & \multicolumn{1}{c|}{$\boldsymbol{n}$} & \multicolumn{1}{c|}{$\boldsymbol{m}$} & \multicolumn{1}{c|}{\bf Type}  & \multicolumn{1}{c|}{\bf Linking Site}\\
%    \hline
    \hline
    {\em DBLP}   &613.6K    & 2.0M          & undirected & www.dblp.com\\% 1 \\
    \hline
    {\em Web-St}      & 281.9K    & 2.3M      & directed & www.stanford.edu\\
    \hline
    {\em Pokec}      & 1.6M    &30.6M      & directed & pokec.azet.sk \\
    \hline
    {\em LJ} & 4.8M & 69.0M    & directed &  www.livejournal.com \\
    \hline
    {\em Orkut}      & 3.1M    & 117.2M      & undirected  & www.orkut.com \\
    \hline
    {\em Twitter}   & 41.7M & 1.5B & directed & twitter.com\\
    \hline\hline
    {\em RMAT-1}   & 1.6M    &30.6M      & directed & -\\
    \hline
    {\em RMAT-2}   & 3.1M    & 117.2M      & directed  & -\\
    \hline
    {\em RMAT-3}   & 41.7M & 1.5B & directed & -\\
    \hline
    {\em RMAT-4}   & 128M & 8.6B & directed & -\\
  


    \hline\hline
    {\em X0}   & 26.1M & 485.6M  & undirected & x.com\\
    \hline
    {\em X1}   &50.1M & 792.0M & undirected & x.com\\
    \hline
    {\em X2}   &58.2M & 1.1B & undirected & x.com\\
    \hline
    {\em X3}   & 74.3M & 1.5B & undirected & x.com\\
  \hline

   %{\em X3}   & 219.6M & 5.6B & undirected & x.com\\
   %\hline
\end{tabular}%}
\end{table}


%\vspace{-2mm}
\subsection{Experimental Settings}


%\header
{\bf Datasets and query sets.} We use 6 real graphs: {\em DBLP}, {\em Web-St}, {\em Pokec},  {\em LJ}, {\em Orkut}, and {\em Twitter}, which are public benchmark datasets used in recent work \cite{lofgren2015personalized,WangTXYL16}. We further generate four synthetic datasets using the RMAT random graph generator \cite{ChakrabartiZF04}, denoted as RMAT1, RMAT2, RMAT3, and RMAT4, to examine the scalability of our proposed top-$k$ algorithms. Note that the largest synthetic dataset RMAT includes 8.6 billion edges. We further test our methods on  four user networks from company X \footnote{Anonymized due to double-blind submission.}. Table \ref{tbl:exp-data} summarizes the statistics of the datasets. For each dataset, we choose $50$ source nodes uniformly at random, and we generate an SSPPR query from each chosen node. In addition, we also generate $5$ top-$k$ queries from each source node, with $k$ varying in $\{100, 200, 300, 400, 500\}$. Note that the maximum $k$ is set to $500$ in accordance to Twitter's Who-To-Follow service \cite{gupta2013wtf}, whose first step requires deriving top-$500$ PPR results.

\header
{\bf Methods.} For whole-graph SSPPR queries, we compare our proposed {\em \ssppr} and {\em \ssppr+} against three methods: (i) the {\em Monte-Carlo} approach, dubbed as {\em MC}; (ii) the optimized {\em BiPPR} for SSPPR queries described in Section \ref{app:ssbippr}; (iii) {\em HubPPR}, which is the indexed version of {\em BiPPR}.
We further compare our {\em FORA} and {\em FORA+} against the version without the optimization techniques (Ref. Section \ref{sec:opt}), dubbed as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based methods, respectively. 

For top-$k$ SSPPR queries, we compare our algorithm with the existing approximate solutions: the single-source {\em BiPPR}, the top-$k$ algorithm for {\em HubPPR} in \cite{WangTXYL16}, and the {\em TopPPR} \cite{WeiHX0SW18}. For {\em BiPPR} and {\em HubPPR}, we use the same $\epsilon$, $\delta$, and $\pf$ as FORA. For {\em TopPPR}, we follow the settings in \cite{WeiHX0SW18} and set $\rho=0.99$. We further extend our top-$k$ algorithm (Ref. Algorithm \ref{alg:layer-topk}) to the Monte-Carlo approach, and denote this algorithm as {\em MC-Topk}. We also include the {\em Forward Push} \cite{AndersenCL06} and {\em TPA} \cite{yoon2018tpa} as a baseline for top-$k$ SSPPR queries, and we tune their accuracy control parameters on each dataset separately, so that their precisions for top-$k$ PPR queries are the same as {\em \ssppr} on each dataset. Besides, we also compare our {\em FORA} and {\em FORA+} against the version without the top-$k$ optimization techniques (Ref. Section \ref{sec:topk-running-time-guarantee}), dubbed as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based algorithms, respectively.


\header
{\bf Parameter setting.} Following previous work \cite{lofgren2014fast,lofgren2015personalized,WangTXYL16}, we set $\delta = 1/n, \pf = 1/n$, and $\eps=0.5$. %For {\em HubPPR}, the index size is set to the same as {\em \ssppr+}.
For our {\em FORA} and {\em FORA+}, note that the performance and / or the index size depends on the choice of $\rmax$. For the whole-graph queries, we will use the balanced strategy to auto-decide the choice of $\rmax$ for {\em FORA} and build the index based on the strategy as mentioned in Section \ref{sec:opt-balanced}. For {\em FORA-Basic} and {\em FORA-Basic+}, $\rmax$ is set according to Section \ref{sec:ana}, and the index is built based on the chosen $\rmax$. For top-$k$ PPR query, the index size cannot be auto-decided using our balancing strategy since the top-$k$ algorithm is more complicated and involving. Therefore, we will tune $\rmax$ to find the best index size for our top-$k$ queries. In particular, we set $\rmax$ according to Section \ref{sec:ana}, denote the value as $\rmax^*$, and then set $\rmax$ to $\rmax^*$, $3\rmax^*$, $5\rmax^*$, and $7\rmax^*$. As we show in the experiment, when $\rmax$ is set to $\rmax^*$, it achieves the best trade-off, and therefore we use this setting in our top-$k$ evaluation.
For fair comparison, the index size of {\em HubPPR} is set to be the same as that of {\em \ssppr+} for top-$k$ SSPPR processing and also {\em \ssppr-Origin+} (for whole-graph SSPPR processing).

%Note that there is a trade-off between the query efficiency and the precision of the top-$k$ PPR query when we choose $\rmax$ (Refer Section \ref{sec:existingsolutions} for the definition of $\rmax$) for the {\em Forward Push} algorithm. We tune the parameter of its $\rmax$ so that the precision of the {\em Forward Push} algorithm is the same as {\em \ssppr} for the top-500 SSPPR queries.



\subsection{Whole-Graph SSPPR Queries} \label{sec:exp-ss}


In our first set of experiments, we evaluate the efficiency of each method for whole-graph SSPPR queries on the 6 public datasets.
%We include four variants of our proposed methods. We denote our implementation without optimization techniques (Ref. Section \ref{sec:opt}) as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free method and index-based method, respectively. For the versions with optimizations, we denote them as {\em FORA} and {\em FORA+} for the index-free and index-based methods, respectively.
Table \ref{tbl:ppr-query} reports the average query time of each method. Observe that both {\em \ssppr} and {\em BiPPR} achieve better query performance than {\em MC}, which is consistent with our analysis that the time complexity of {\em \ssppr} and {\em BiPPR} is better than that of {\em MC}. Moreover, {\em \ssppr} is at least $4$ times faster than {\em BiPPR} on most of the datasets. %For instance, on Twitter, {\em \ssppr} is around 3.7x faster than {\em BiPPR}.
The reason, as we explain in Section \ref{sec:ana}, is that {\em BiPPR} either degrades to the {\em MC} approach when the backward threshold is large, or requires conducting a backward search from each node $v$ in $G$, even if $\pi(s, v)$ is extremely small. In contrast, {\em \ssppr} avoids degrading to {\em MC} and tends to omit nodes with small PPR values, which helps improve efficiency. In addition, {\em \ssppr+} achieves significant speedup over {\em \ssppr}, and is around 10 times faster than the latter on most of the datasets. %This is due to our advanced design of the index structure according to our theoretical analysis in Section \ref{sec:ana}.
The {\em HubPPR} also improves over {\em BiPPR}, but the improvement is far less than what {\em \ssppr+} achieves over {\em \ssppr}. %The reason is that, for single-source PPR queries, the number of required random walks is much larger than that in point-to-point PPR queries. Hence, when the stored random walks are consumed on a hub, and it needs to do random walks online.
Moreover, even without any index, {\em \ssppr} is still more efficient than {\em HubPPR}. %which indicates that the proposed {\em \ssppr} is more favorable choice on single-source PPR queries than other alternatives.

As we can observe from Table \ref{tbl:ppr-query}, with our optimization techniques introduced in Section \ref{sec:opt}, the index-free method {\em FORA} improves over {\em FORA-Basic} by up to 1.8x. Apart from the 6 public datasets, we further test the effectiveness of our methods on the four social networks from company X. We omit the results for the baseline methods (MC, BiPPR, and HubPPR) since they incur prohibitive processing costs.  As shown in Table \ref{tbl:fora-ss-opt}, {\em FORA} still improves over {\em FORA-Basic} by more than 2x almost on all datasets, which demonstrates the effectiveness of our proposed optimization technique for online algorithms. For the index-based method, {\em FORA} improves over {\em FORA+} by at least twice on almost all datasets, and up to 2.8x. As shown in Table \ref{tbl:exp-space-consumption},  the space consumption required by {\em FORA+} is twice as that of {\em FORA-Basic+}, which demonstrates that our optimization technique achieves a good trade-off between query time and space consumption.

%\begin{table}[!t]
%\centering
%\tbl{Whole-graph SSPPR performance (s). ($K=10^3$) \label{tbl:ppr-query}}{
%  \begin{tabular}{ | l | r | r|r|r |r|r|r|}
%    \hline
%        & {\em MC} & {\em BiPPR} & {\em HubPPR}&   {\em \ssppr} & {\em \ssppr-OPT} & {\em \ssppr+} & {\em \ssppr-OPT+}\\
%    \hline
% {\em DBLP}  &14.2 &	3.8&  	2.8&	0.8& 0.6	& 0.09 & 0.05  \\
%    \hline
%{\em Web-St}  & 5.4	&3.7&  	1.6	&0.03& 0.02	&  0.01& 0.01 \\
%    \hline
% {\em Pokec} &69.1	&24.9& 19.6& 11.26&	6.3 & 0.9 & 0.4 \\
%    \hline
% {\em LJ}&163.5	& 61.4& 50.8	& 15.5 & 9.9	&1.2 & 0.6 \\
%    \hline
%{\em Orkut} &230.6	& 158.2 &126.3	& 40.1& 26.4	& 4.8	& 1.7 \\
%    \hline
%{\em Twitter}   &4.3K	&3.1K& 	 2.4K & 513.8& 283.1	&63.3 &	 29.8\\
%    \hline \hline
%{\em X0}   & 2.4K	&  & 	 &  & 	&66.7 &	 \\
%    \hline
%{\em X1}   &5.3K	& & 	 &  & 	&130.7 &	 \\
%    \hline
%{\em X2}   &	& & 	 &  & 	& 152.4 &	 \\
%    \hline
%{\em X3}   &	& & 	 &  & 	&216.8 &	 \\
%    \hline
%  \end{tabular}}
%\end{table}

\begin{table}[!t]
\centering
%\tbl{Whole-graph SSPPR performance (s) (i). ($K=10^3$) \label{tbl:ppr-query}}{
\caption{Whole-graph SSPPR performance (s) (i). ($K=10^3$)}
\label{tbl:ppr-query}
  \begin{tabular}{ | l | r | r|r|r |r|r|r|}
    \hline
        & {\em MC} & {\em BiPPR} & {\em HubPPR} & {\em FORA-Basic} & {\em FORA} & {\em FORA-Basic+}&   {\em \ssppr+} \\
    \hline
 {\em DBLP}  &14.2 &	3.8&  	2.8&	0.8& 0.6	& 0.09 & 0.05 \\
    \hline
{\em Web-St}  & 5.4	&3.7&  	1.6	& 0.03& 0.02	&  0.01& 0.01 \\
    \hline
 {\em Pokec} &69.1	&24.9& 19.6& 11.26&	6.3 & 0.9 & 0.4	 \\
    \hline
 {\em LJ}&163.5	& 61.4& 50.8	& 15.5 & 9.9	&1.2 & 0.6 \\
    \hline
{\em Orkut} &230.6	& 158.2 &126.3	&  40.1& 26.4	& 4.8	& 1.7 \\
    \hline
{\em Twitter}   &4.3K	&3.1K& 	 2.4K &  513.8& 283.1	&63.3 &	 29.8\\
    \hline
  \end{tabular}%}
\end{table}




\begin{table}[!t]
\centering
%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
\caption{Whole-graph SSPPR performance (s) (ii). ($K=10^3$)}
\label{tbl:fora-ss-opt}
  \begin{tabular}{ | l | r | r|r|r|}
    \hline
        & {\em FORA-Basic} & {\em FORA} & {\em FORA-Basic+}&   {\em \ssppr+}\\
    \hline
{\em X0}   & 527.47  & 259.9	&66.7 &	31.2 \\
    \hline
{\em X1}   & 957.4 &  504.9 	&130.7 &	60.4 \\
    \hline
{\em X2}   & 1072.5 & 530.4	& 152.4 &	63.7 \\
    \hline
{\em X3}   & 2340.6 &  1163.3 	&216.8 & 97.2	 \\
    \hline
  \end{tabular}%}
\end{table}












\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{small}
    \begin{tabular}{cc}
        %\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
      	\multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\
      	
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/dblp-topk-time.eps} &
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/pokec-topk-time.eps} \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/dblp-topk-time.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/pokec-topk-time.eps} \\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\%[-1mm]

        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/orkut-topk-time.eps} &
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/tw-topk-time.eps} \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/orkut-topk-time.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/tw-topk-time.eps} \\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\%[-1mm]

 \end{tabular}
 \caption{Top-$k$ SSPPR query efficiency: varying $k$.} \label{exp:topk-time}
\end{small}
\end{figure*}
\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
\begin{small}
    \begin{tabular}{cc}
        %\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
        \multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\

%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/dblp-topk-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/pokec-topk-prec.eps}\\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/dblp-topk-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/pokec-topk-prec.eps}\\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/orkut-topk-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/tw-topk-prec.eps}\\
	 	\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/orkut-topk-prec.eps} &
		\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/tw-topk-prec.eps}\\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\
 \end{tabular}
 \caption{Top-$k$ SSPPR query accuracy: varying $k$.} \label{exp:topk-acc}
\end{small}
\end{figure*}

\begin{figure*}[!t]
	\centering
	%\vspace{-2mm}
	\begin{small}
		\begin{tabular}{cc}
			%\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
			\multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\

			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/dblp-topk-prec.eps} &
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/pokec-topk-prec.eps}\\
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/dblp-topk-ndcg.eps} &
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/pokec-topk-ndcg.eps}\\
			\hspace{-2mm} (a) DBLP  &
			\hspace{-2mm} (b) Pokec \\
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/orkut-topk-prec.eps} &
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/tw-topk-prec.eps}\\
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/orkut-topk-ndcg.eps} &
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/tw-topk-ndcg.eps}\\
			\hspace{-2mm} (c) Orkut &
			\hspace{-2mm} (d) Twitter \\
		\end{tabular}
		\caption{Top-$k$ SSPPR query NDCG: varying $k$.} \label{exp:topk-ndcg}
	\end{small}
\end{figure*}



\begin{table}[!t]
	\centering
	%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
	\caption{Running time on RMAT. ($K=500$)}
	\label{tbl:rmat-runningtime}
	\begin{tabular}{ | l | r | r|r|r|}
		\hline
		& {\em RMAT-1} & {\em RMAT-2} & {\em RMAT-3}&   {\em RMAT-4}\\
		\hline
		{\em FORA+}   & 0.729 & 0.9944	& 0.999901 &	618MB \\
		\hline
		{\em TopPPR}   & 1.36431&  0.9946	&0.999917 & 259MB	 \\
		\hline
	\end{tabular}%}
\end{table}

\begin{table}[!t]
	\centering
	%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
	\caption{Performance (s) on RMAT-2. ($K=500$)}
	\label{tbl:rmat-2}
	\begin{tabular}{ | l | r | r|r|r|}
		\hline
		& {\em Running time} & {\em Precision} & {\em NDCG}&   {\em Memory Usage}\\
		\hline
		{\em FORA+}   & 4.69827 & 0.9957	& 0.999865 &	2.02GB \\
		\hline
		{\em TopPPR}   &5.07309&  0.996	&0.999941 & 1.79GB	 \\
		\hline
	\end{tabular}%}
\end{table}

\begin{table}[!t]
	\centering
	%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
	\caption{Performance (s) on RMAT-3. ($K=500$)}
	\label{tbl:rmat-3}
	\begin{tabular}{ | l | r | r|r|r|}
		\hline
		& {\em Running time} & {\em Precision} & {\em NDCG}&   {\em Memory Usage}\\
		\hline
		{\em FORA+}   & 17.4335 & 0.9931	& 0.999883 &	20.08GB \\
		\hline
		{\em TopPPR}   & 51.1156&  0.9936	&0.99993 & 11.56GB	 \\
		\hline
	\end{tabular}%}
\end{table}

\begin{table}[!t]
	\centering
	%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
	\caption{Performance (s) on RMAT-4. ($K=500$)}
	\label{tbl:rmat-4}
	\begin{tabular}{ | l | r | r|r|r|}
		\hline
		& {\em Running time} & {\em Precision} & {\em NDCG}&   {\em Memory Usage}\\
		\hline
		{\em FORA+}   &149.473 & 0.9954	& 0.99996 &	96.25GB \\
		\hline
		{\em TopPPR}   & 481.002&  0.9951	&0.999824& 66.00GB	 \\
		\hline
	\end{tabular}%}
\end{table}

%\vspace{-1mm}
\subsection{Top-$\boldsymbol k$ SSPPR Queries} \label{sec:exp-topk}
%$This section evaluates the efficiency and accuracy of the proposed top-$k$ PPR query algorithms against the states-of-the-art.
%
In our second set of experiments, we evaluate the efficiency and accuracy of each method for top-$k$ SSPPR queries. For our methods, we only include our {\em FORA} and {\em FORA+} that includes the optimizations presented in Section \ref{sec:topk-running-time-guarantee} to avoid the figures being too crowded. We will examine the effectivess of our optimization techniques in the next set of experiments.


{\cblue
\subsubsection{Top-$\boldsymbol k$ query efficiency}

Figures \ref{exp:topk-time} reports the average query time of each method on four representative datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, and {\em Twitter}. (The results on the other two datasets are qualitatively similar, and are omitted due to the space constraint.) Note that the y-axis is in log-scale. 
Recall that {\em Forward Push} provides no approximation guarantee, and we tune the $\rmax$ on each dataset separately, so that it provides the same precision for top-500 SSPPR queries as our {\em \ssppr} algorithm does. Similarly, for TPA \cite{yoon2018tpa}, we tune their parameters so that it provides the best possible precision.

The main observation is that our {\em \ssppr+} achieves the best performance on all the datasets. For instance, on Twitter dataset with $k=500$, our {\em \ssppr+} provides similar or better accuracy and NDCG as competitors, and runs 2x faster than TopPPR, two order of magnitude faster than MC-Topk, and more than 500x faster than Forward Push, TPA, BiPPR, and HubPPR. 
This is expected since our FORA+ applies an iterative approach to refine the top-$k$ answers and terminates immediately whenever the answer could provide the desired approximation guarantee; it further uses the indexing scheme to reduce the expensive costs of random walks.

Our FORA is the fastest online algorithm except TopPPR since TopPPR uses a more advanced filter-refinement paradigm to answer the top-$k$ queries. However, their proposed approach does not benefit from indexing scheme, and is outperformed by our FORA+. It is also difficult for TopPPR to benefit from indexing scheme since {\em (i)} their random walk adopts the $\sqrt{\alpha}$-random walk, and all the nodes visited will be used to estimate the PPR scores; {\em (ii)} the sources of random walks in Monte-Carlo phase are generated randomly in TopPPR and it may results in poor cache performances. In contrast, FORA+ only need to scan the index structures in order and only stores the destinations in index structure, making it light-weighted and cache-friendly.

Another observation is that after extending the MC approach with our top-$k$ algorithm, MC-Topk achieves more than 20x speedup on Twitter over its single-source alternative. This further demonstrates the effectiveness of our top-$k$ algorithm proposed in Section \ref{sec:topk-running-time-guarantee}, which improves the time complexity to $O(\frac{\log{n}}{\epsilon^2\cdot \pi(s,v_k^*)})$. However, our FORA and FORA+ are still far more efficient than MC-Topk since FORA and FORA+ explores the forward push to reduce the random walk costs.


%Recall that {\em Forward Push} provides no approximation guarantee, and we tune the $\rmax$ on each dataset separately, so that it provides the same precision for top-500 SSPPR queries as our {\em \ssppr} algorithm does. Similarly, for TPA \cite{yoon2018tpa}, we tune their parameters so that it provides the same precision as our methods.

%Observe that, when both algorithms provide the identical precision, the performance of the proposed {\em \ssppr} and {\em Forward Push} is roughly comparable on small and medium size graphs, e.g., on {\em DBLP}, {\em Pokec}, and {\em Orkut}. When the graph size increases, however, {\em \ssppr} dominates the {\em Forward Push} in terms of the query efficiency. In particular, on {\em Twitter}, {\em \ssppr} is faster than {\em Forward Push} by two orders of magnitude. Compared with {\em TPA}, our proposed {\em \ssppr} still outperforms it by up to two order of magnitude when providing identical precision.

Finally, with our index structure, {\em \ssppr+} further improves over {\em \ssppr} by an order of magnitude, which demonstrates the effectiveness of the index structure. Notably, on the Twitter social network with 1.5 billion edges, our {\em FORA+} can answer the top-500 query in 0.8 second.

%{\em Forward Push} is practically efficient on small graphs, e.g., {\em DBLP} and {\em Pokec}, and can even outperform the proposed {\em \ssppr} on large $k$ settings, e.g., when $k=400$. However, on large graphs, the proposed {\em \ssppr} is more efficient than the Forward Push algorithm, and improves over the Forward Push algorithm by up to an order of magnitude on the Twitter dataset. Moreover, our {\em \ssppr} provides strict approximation guarantee for the top-$k$ SSPPR query, while the {\em Forward Push} provides no guarantee on the results. This indicates that our {\em \ssppr} is a preferred choice

%This indicates that our {\em \ssppr} achieves a better trade-off among the theoretical guarantee, the practical query accuracy and time efficiency than the {\em Forward Push} algorithm.



%The reason is that {\em HubPPR} requires performing a large number of backward searches, as is the case for {\em BiPPR}.
%
%%Nevertheless, even without index, our {\em \ssppr} is still several times faster than {\em HubPPR}. With full-fledged index, our {\em \ssppr+} is an order of magnitude faster than {\em HubPPR} approach.
%
\subsubsection{Top-$\boldsymbol k$ query accuracy}

To compare the accuracy of the top-$k$ results returned by each method, we first calculate the ground-truth answer of the top-$k$ queries using the {\em Power Iteration} \cite{page1999pagerank} method with 100 iterations. Afterwards, we evaluate the top-$k$ results of each algorithm by their precision and NDCG \cite{JarvelinK00} with respect to the ground truth. 
Note that the precision and recall are the same for the top-$k$ SSPPR queries, and is the fraction of nodes returned by the top-$k$ algorithm that are real top-$k$ nodes.  For NDCG, let $s$ be the query node, $v_1,v_2,\cdots, v_k$ be the $k$ nodes returned by the top-$k$ algorithm, and $v_1^*, v_2^*,\cdots, v_k^*$ be the true top-$k$ nodes. Then, the NDCG is defined as $\frac{1}{Z_k}\sum_{i=1}^k{\frac{2^{\pi(s,v_i)}-1}{\log{(i+1)}}}$, where $Z_k=\sum_{i=1}^k{\frac{2^{\pi(s,v_k^*)-1}}{\log{(i+1)}}}$.


Figure~\ref{exp:topk-acc} (resp. Figure~\ref{exp:topk-ndcg}) show the accuracy (resp. NDCG) of the top-$k$ query algorithms on four datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, and {\em Twitter}. Observe that all methods except TPA consistently provide high precisions and all methods achieve very high NDCG (all above 0.999). In the meantime, notice that our FORA+ is consistently similar precision as TopPPR on all the tested datasets.

%To explain, all these four algorithms include a local update algorithm, either forward push or backward push, and provides a deterministic part, i.e., $\rese(s,v)$, and then use random walks to approximate the remaining part. However, the {\em MC} approach only use the random walks to estimate the PPRs, which is less accurate than the other solutions.
}







\subsection{Effectiveness of the Top-$\boldsymbol k$ optimization}
In this set of experiment, we evaluate the effectiveness of the new top-$k$ algorithm proposed in Section \ref{sec:topk-running-time-guarantee}, which provides improved time complexity, and reduces the time to calculate the bounds for each node. We present the results for 6 representative datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, {\em Twitter}, {\em X2}, and {\em X3}.

Figures \ref{exp:top-opt-time}(a)-(f) demonstrate the running time of {\em FORA} and {\em FORA+}, against the versions without the optimization techniques in Section \ref{sec:topk-running-time-guarantee}, referred to as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based solution, respectively. As we can observe, with the new algorithm, {\em FORA} (resp. {\em FORA+} improves over {\em FORA-Basic} (resp. {\em FORA-Basic+}) by a large margin. For instance, on Twitter dataset, {\em FORA} (resp. {\em FORA+}) improves over {\em FORA-Basic} (resp. {\em FORA-Basic+}) by around 4x (resp. 6x). The main reason for the significant improvement are two-fold: (i) the time complexity of {\em FORA} and {\em FORA+} depend on $\frac{1}{\pi(s,v^*_k)}$ while {\em FORA-Basic} and {\em FORA-Basic+} depend on $\frac{1}{n}$; (ii) {\em FORA} and {\em FORA+} avoids the expensive bound calculation part that are required by {\em FORA-Basic} and {\em FORA-Basic+}.

Next, we report the accuracy of the four methods on the 6 datasets as shown in Figures \ref{exp:top-opt-acc}(a)-(f). As we can observe, all four methods provide similarly high accuracy for the top-$k$ queries on all datasets. To explain, all four methods share the similar spirit by adaptively refine the top-$k$ answer and return the approximate answer with theoretical guarantees. Therefore, all the four methods provide similarly high accuracy.




\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{small}
    \begin{tabular}{cc}
          \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/topk-opt/topk-opt-algo-legend.eps}}  \\[0mm]
      %\multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figs/topk_query_legend.eps}}  \\[-2mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-dblp.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-pokec.eps} \\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\%[-1mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-orkut.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-twitter.eps} \\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\%[-1mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x2.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x3.eps} \\
        \hspace{-2mm} (e) X2 &
        \hspace{-2mm} (f) X3 \\%[-1mm]

 \end{tabular}
 \caption{Effectiveness of top-$k$ Optimization: query efficiency.} \label{exp:top-opt-time}
\end{small}
\end{figure*}

\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
\begin{small}
    \begin{tabular}{cc}
      \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/topk-opt/topk-opt-algo-legend.eps}}  \\[0mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-dblp-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-pokec-prec.eps}\\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-orkut-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-twitter-prec.eps}\\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x2-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x3-prec.eps}\\
        \hspace{-2mm} (e) X2 &
        \hspace{-2mm} (f) X3 \\
 \end{tabular}
 \caption{Effectiveness of top-$k$ Optimization: query accuracy.} \label{exp:top-opt-acc}
\end{small}
\end{figure*}






%\begin{figure*}[!t]
% \centering
%   %\vspace{-2mm}
%    \begin{small}
%    \begin{tabular}{cc}
%          \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
%      %\multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figs/topk_query_legend.eps}}  \\[-2mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-dblp.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-pokec.eps} \\
%        \hspace{-2mm} (a) DBLP  &
%        \hspace{-2mm} (b) Pokec \\%[-1mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-orkut.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-twitter.eps} \\
%        \hspace{-2mm} (c) Orkut &
%        \hspace{-2mm} (d) Twitter \\%[-1mm]
%
% \end{tabular}
% \caption{Top-$k$ SSPPR query efficiency: varying $\epsilon$.} \label{exp:2topk-time}
%\end{small}
%\end{figure*}
%
%\begin{figure*}[!t]
% \centering
%   %\vspace{-2mm}
%\begin{small}
%    \begin{tabular}{cc}
%      \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-dblp-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-pokec-prec.eps}\\
%        \hspace{-2mm} (a) DBLP  &
%        \hspace{-2mm} (b) Pokec \\
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-orkut-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-twitter-prec.eps}\\
%        \hspace{-2mm} (c) Orkut &
%        \hspace{-2mm} (d) Twitter \\
% \end{tabular}
% \caption{Top-$k$ SSPPR query accuracy: varying $\epsilon$.} \label{exp:2topk-acc}
%\end{small}
%\end{figure*}




%\vspace{-2mm}
\subsection{Preprocessing Costs}\label{sec:exp-preprocessing}


\begin{table}[!t]
\vspace{0mm}
\centering
%\hspace*{-3mm}
%\tbl{Preprocessing time.\label{tbl:exp-preprocessing-time}}{
\caption{Preprocessing time.}
\label{tbl:exp-preprocessing-time}
  \begin{tabular}{ | p{0.6in} | p{0.6in} |p{0.4in}|p{0.8in}|p{1.3in} |}
    \hline
     {\bf Datasets}  & {\em HubPPR}& {\em TPA} & {\em \ssppr+ (for whole graph)} &{\em \ssppr-Basic+} \& {\em \ssppr+ (for top-$k$)} \\
    \hline
 {\em DBLP} & 26.4& 4.4 & 7.6	& 3.6	  \\
    \hline
{\em Web-St}  &  9.3& 1.3 & 3.2 &1.5  \\
    \hline
 {\em Pokec} &90.6& 42.5 & 77.1	&34.6 \\
    \hline
 {\em LJ}& 279.9& 112.5 & 181.3	&81.2   \\
    \hline
{\em Orkut} &530.6& 177.3& 383.5 & 165.9\\
    \hline
{\em Twitter}   &5088.6& 3112.3 & 5130.4	& 2255.4	\\
    \hline\hline
{\em X0}   &-&- & 2031.2	&967.14	\\
\hline
{\em X1}   &-&- & 5244.5	& 2428.6	\\
\hline
{\em X2}   &-&- & 5721.7	& 2602.9	\\
\hline
{\em X3}   &-&- & 8836.4	& 4213.5	\\
\hline
  \end{tabular}%}
\end{table}

Finally, we inspect the preprocessing costs of our methods against alternatives. We first examine the preprocessing time of the index-based methods: {\em \ssppr+}, {\em \ssppr-Origin+}, {\em HubPPR}, and {\em TPA}. Note that the $\rmax$ of {\em FORA+} for whole-graph and top-$k$ queries are different, and therefore the preprocessing time are shown as seperately in Table \ref{tbl:exp-preprocessing-time}. The choice of tuned $\rmax$ of {\em FORA+} is the same as that of {\em FORA-Basic}, and therefore their preprocessing time are the same.
As shown in Table \ref{tbl:exp-preprocessing-time}, the preprocessing time of {\em \ssppr+}, {\em FORA-Basic+}, {\em HubPPR}, and {\em TPA} are all moderate. On the largest dataset {\em X3}, our {\em FORA+} for whole graph SSPPR queries (resp. for top-$k$ SSPPR queries) can still finish index construction in less than 3 hours (resp. less than 1 and half an hour), which is more than compensated by its high query performance as shown in Table \ref{tbl:ppr-query}. Besides, this preprocessing time can be further significantly reduced by parallelizing the index construction process.




\begin{table}[!t]
\vspace{0mm}
\centering
%\hspace*{-3mm}
%\tbl{Space consumption.\label{tbl:exp-space-consumption}}{
\caption{Space consumption.}
\label{tbl:exp-space-consumption}
  \begin{tabular}{|  p{0.6in}|p{0.7in}| p{0.4in} |p{0.4in}|p{0.4in}|p{1.4in}|p{0.8in} |}
    \hline
      {\bf Datasets}   & {\em MC} \& {\em FORA} & {\em BiPPR}&{\em HubPPR} & {\em TPA} &  {\em FORA-Basic+} \& {\em FORA+} (for top-$k$) & {\em FORA+} (for whole-graph) \\
    \hline
 {\em DBLP} & 18.4MB &	36.8MB& 127.6MB	&23.3MB	& 109.2MB & 200.1MB \\
    \hline
{\em Web-St}  &  10.4MB & 20.8MB& 66.3MB  &12.6MB	& 55.9MB& 101.4MB \\
    \hline
 {\em Pokec} &130.8MB &	261.5MB & 673.5MB &143.6MB	& 542.7MB& 954.6MB\\
    \hline
 {\em LJ}& 295.2MB	&590.5MB & 1.7GB &333.6MB	&1.4GB & 2.5GB \\
    \hline
{\em Orkut} &950.1MB	&1.9GB& 3.5GB &974.9MB	& 2.6GB& 4.2GB \\
    \hline
{\em Twitter}   &6.2GB &12.5GB&  25.1GB	&6.5GB& 18.8GB & 31.4GB	\\
    \hline\hline
{\em X0} &  2.0GB	&-& - &-	& 7.5GB& 13.1GB \\
    \hline
{\em X1} &3.2GB	&-& - &-	& 13.2GB& 23.2GB \\
    \hline
{\em X2} &4.6GB	&-& - &-	& 17.5GB& 30.4GB \\
    \hline
{\em X3} & 6.0GB	&-& - &-	& 22.6GB& 39.2GB \\
    \hline
  \end{tabular}%}
\end{table}


Next, we examine the space consumption of all methods. Note that each method will need to store at least a copy of the graph. For {\em MC}, {\em FORA}, and {\em TPA}, they can store only a single copy of the input graph (each node stores the out-neighbor list). However, for {\em HubPPR} and {\em BiPPR}, they need to store two copies of the graph (each node stores an out-neighbor and an in-neighbor list) for efficient random walks and backward propagation.

Table \ref{tbl:exp-space-consumption} reports the space consumption of all methods. As we can observe, the index size of our {\em \ssppr+} for whole-graph queries and top-$k$ queries are no more than 7.5x and 4x of the original graph, respectively. The space consumption is more than compensated by the superb performance of {\em FORA+}, where we can answer a whole-graph query within 30 seconds and  top-$k$ query within 1 second on the 1.5 billion edge Twitter graph, which improves over the index-free {\em FORA} by more than an order of magnitude on almost all datasets. This demonstrates the effectiveness and efficiency of our indexing scheme. Besides, even without index, our {\em FORA} can still outperform all alternative index-free and index-based methods on whole-graph SSPPR queries and  top-$k$ SSPPR queries by a large margin. The experimental results demonstrate that our proposed methods achieve a good trade-off between the space consumption and query efficiency when providing query answers with identical accuracy.



\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{tabular}{cc}
    \hspace{-4mm} \includegraphics[height=2.4mm]{./figure/topk-tune-rmax/tune-rmax-legend1.eps} & \hspace{8mm}\includegraphics[height=2.4mm]{./figure/topk-tune-rmax/tune-rmax-legend2.eps} \\[0mm]
        \hspace{-4mm}  \includegraphics[height=35mm]{./figure/topk-tune-rmax/rmax-vs-query1.eps} &
         \hspace{8mm} \includegraphics[height=35mm]{./figure/topk-tune-rmax/rmax-vs-query2.eps}\\
        \hspace{-4mm} (a)   &
        \hspace{8mm}(b)  \\

 \end{tabular}
 \caption{Tunning $\rmax$ for top-$k$ SSPPR queries ($\times\rmax^*$)}. \label{exp:top-tune-rmax}
\end{figure*}





Finally, we examine the trade-off between the space consumption and top-$k$ query performance of our {\em FORA+} algorithm by tuning $\rmax$.  Let $\rmax^*$ be the $\rmax$ value set according to Section \ref{sec:ana}. We then set $\rmax$ to $\rmax^*$, $3\rmax^*$, $5\rmax^*$, and $7\rmax^*$. Notice that, the index size is proportional to $\rmax$ and let $y$ be the index size when $\rmax = \rmax^*$. Then, the index size will be $y$, $3y$, $5y$, and $7y$, respectively. As we can observe, when we increase the index size for {\em FORA+}, the query performance also improves on almost all datasets. To explain, by increasing the index size, {\em FORA+} avoids the expensive random walks and thus saving the query time. However, from the experiment, we can observe that when $\rmax = \rmax^*$, it actually achieves the best trade-off between the query performance and space consumption, and hence in our experiment, we set $\rmax=\rmax^*$ for all the top-$k$ queries.


==> 6-Exp/exp__Wang_Sibo_________________2019-03-14_.tex <==
%!TEX root=../ssppr_kdd17_newformat.tex

\section{Experiments} \label{sec:exp}

In this section, we experimentally evaluate our methods for whole-graph SSPPR queries and top-$k$ SSPPR queries. For whole-graph (resp. top-$k$) SSPPR queries, we include our index free methods {\em \ssppr}, which includes the optimizations as mentioned in Section \ref{sec:opt} (resp. Section \ref{sec:topk-running-time-guarantee}),  and their index-based variant, referred to as {\em \ssppr+}, against the states of the art. All experiments are conducted on a Linux machine with an Intel 2.9GHz CPU and 200GB memory.

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
%\tbl{Datasets. ($K=10^3, M=10^6, B=10^9$\label{tbl:exp-data})}{
\caption{Datasets. ($K=10^3, M=10^6, B=10^9$)}
\label{tbl:exp-data}
\begin{tabular}{|l|r|r|r|c|}
    \hline
    {\bf Name} & \multicolumn{1}{c|}{$\boldsymbol{n}$} & \multicolumn{1}{c|}{$\boldsymbol{m}$} & \multicolumn{1}{c|}{\bf Type}  & \multicolumn{1}{c|}{\bf Linking Site}\\
%    \hline
    \hline
    {\em DBLP}   &613.6K    & 2.0M          & undirected & www.dblp.com\\% 1 \\
    \hline
    {\em Web-St}      & 281.9K    & 2.3M      & directed & www.stanford.edu\\
    \hline
    {\em Pokec}      & 1.6M    &30.6M      & directed & pokec.azet.sk \\
    \hline
    {\em LJ} & 4.8M & 69.0M    & directed &  www.livejournal.com \\
    \hline
    {\em Orkut}      & 3.1M    & 117.2M      & undirected  & www.orkut.com \\
    \hline
    {\em Twitter}   & 41.7M & 1.5B & directed & twitter.com\\
    \hline\hline
%    {\em RMAT-1}   & 1.6M    &30.6M      & directed & -\\
%    \hline
%    {\em RMAT-2}   & 3.1M    & 117.2M      & directed  & -\\
%    \hline
    {\em RMAT-1}   & 41.7M & 1.5B & directed & -\\
    \hline
    {\em RMAT-2}   & 128M & 8.6B & directed & -\\



    \hline\hline
    {\em X0}   & 26.1M & 485.6M  & undirected & x.com\\
    \hline
    {\em X1}   &50.1M & 792.0M & undirected & x.com\\
    \hline
    {\em X2}   &58.2M & 1.1B & undirected & x.com\\
    \hline
    {\em X3}   & 74.3M & 1.5B & undirected & x.com\\
  \hline

   %{\em X3}   & 219.6M & 5.6B & undirected & x.com\\
   %\hline
\end{tabular}%}
\end{table}


%\vspace{-2mm}
\subsection{Experimental Settings}


%\header
{\bf Datasets and query sets.} We use 6 real graphs: {\em DBLP}, {\em Web-St}, {\em Pokec},  {\em LJ}, {\em Orkut}, and {\em Twitter}, which are public benchmark datasets used in recent work \cite{lofgren2015personalized,WangTXYL16}. We further generate two synthetic datasets using the RMAT random graph generator \cite{ChakrabartiZF04}, denoted as {\em RMAT-1} and {\em RMAT-2} to examine the scalability of our proposed top-$k$ algorithms. Note that {\em RMAT-2} includes 8.6 billion edges. We further test our methods on  four user networks from company X \footnote{Anonymized due to double-blind submission.}. Table \ref{tbl:exp-data} summarizes the statistics of the datasets. For each dataset, we choose $50$ source nodes uniformly at random, and we generate an SSPPR query from each chosen node. In addition, we also generate $5$ top-$k$ queries from each source node, with $k$ varying in $\{100, 200, 300, 400, 500\}$. Note that the maximum $k$ is set to $500$ in accordance to Twitter's Who-To-Follow service \cite{gupta2013wtf}, whose first step requires deriving top-$500$ PPR results.

\header
{\bf Methods.} For whole-graph SSPPR queries, we compare our proposed {\em \ssppr} and {\em \ssppr+} against three methods: (i) the {\em Monte-Carlo} approach, dubbed as {\em MC}; (ii) the optimized {\em BiPPR} for SSPPR queries described in Section \ref{app:ssbippr}; (iii) {\em HubPPR}, which is the indexed version of {\em BiPPR}.
We further compare our {\em FORA} and {\em FORA+} against the version without the optimization techniques (Ref. Section \ref{sec:opt}), dubbed as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based methods, respectively.

For top-$k$ SSPPR queries, we compare our algorithm with the existing approximate solutions: the single-source {\em BiPPR}, the top-$k$ algorithm for {\em HubPPR} in \cite{WangTXYL16}, and the {\em TopPPR} \cite{WeiHX0SW18}. For {\em BiPPR} and {\em HubPPR}, we use the same $\epsilon$, $\delta$, and $\pf$ as FORA. For {\em TopPPR}, we follow the settings in \cite{WeiHX0SW18} and set $\rho=0.99$. We further extend our top-$k$ algorithm (Ref. Algorithm \ref{alg:layer-topk}) to the Monte-Carlo approach, and denote this algorithm as {\em MC-Topk}. We also include the {\em Forward Push} \cite{AndersenCL06} and {\em TPA} \cite{yoon2018tpa} as a baseline for top-$k$ SSPPR queries, and we tune their accuracy control parameters on each dataset separately, so that their precisions for top-$k$ PPR queries are the same as {\em \ssppr} on each dataset. Besides, we also compare our {\em FORA} and {\em FORA+} against the version without the top-$k$ optimization techniques (Ref. Section \ref{sec:topk-running-time-guarantee}), dubbed as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based algorithms, respectively.


\header
{\bf Parameter setting.} Following previous work \cite{lofgren2014fast,lofgren2015personalized,WangTXYL16}, we set $\delta = 1/n, \pf = 1/n$, and $\eps=0.5$. %For {\em HubPPR}, the index size is set to the same as {\em \ssppr+}.
For our {\em FORA} and {\em FORA+}, note that the performance and / or the index size depends on the choice of $\rmax$. For the whole-graph queries, we will use the balanced strategy to auto-decide the choice of $\rmax$ for {\em FORA} and build the index based on the strategy as mentioned in Section \ref{sec:opt-balanced}. For {\em FORA-Basic} and {\em FORA-Basic+}, $\rmax$ is set according to Section \ref{sec:ana}, and the index is built based on the chosen $\rmax$. For top-$k$ PPR query, the index size cannot be auto-decided using our balancing strategy since the top-$k$ algorithm is more complicated and involving. Therefore, we will tune $\rmax$ to find the best index size for our top-$k$ queries. In particular, we set $\rmax$ according to Section \ref{sec:ana}, denote the value as $\rmax^*$, and then set $\rmax$ to $\rmax^*$, $3\rmax^*$, $5\rmax^*$, and $7\rmax^*$. As we show in the experiment, when $\rmax$ is set to $\rmax^*$, it achieves the best trade-off, and therefore we use this setting in our top-$k$ evaluation.
For fair comparison, the index size of {\em HubPPR} is set to be the same as that of {\em \ssppr+} for top-$k$ SSPPR processing and also {\em \ssppr-Origin+} (for whole-graph SSPPR processing).

%Note that there is a trade-off between the query efficiency and the precision of the top-$k$ PPR query when we choose $\rmax$ (Refer Section \ref{sec:existingsolutions} for the definition of $\rmax$) for the {\em Forward Push} algorithm. We tune the parameter of its $\rmax$ so that the precision of the {\em Forward Push} algorithm is the same as {\em \ssppr} for the top-500 SSPPR queries.



\subsection{Whole-Graph SSPPR Queries} \label{sec:exp-ss}


In our first set of experiments, we evaluate the efficiency of each method for whole-graph SSPPR queries on the 6 public datasets.
%We include four variants of our proposed methods. We denote our implementation without optimization techniques (Ref. Section \ref{sec:opt}) as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free method and index-based method, respectively. For the versions with optimizations, we denote them as {\em FORA} and {\em FORA+} for the index-free and index-based methods, respectively.
Table \ref{tbl:ppr-query} reports the average query time of each method. Observe that both {\em \ssppr} and {\em BiPPR} achieve better query performance than {\em MC}, which is consistent with our analysis that the time complexity of {\em \ssppr} and {\em BiPPR} is better than that of {\em MC}. Moreover, {\em \ssppr} is at least $4$ times faster than {\em BiPPR} on most of the datasets. %For instance, on Twitter, {\em \ssppr} is around 3.7x faster than {\em BiPPR}.
The reason, as we explain in Section \ref{sec:ana}, is that {\em BiPPR} either degrades to the {\em MC} approach when the backward threshold is large, or requires conducting a backward search from each node $v$ in $G$, even if $\pi(s, v)$ is extremely small. In contrast, {\em \ssppr} avoids degrading to {\em MC} and tends to omit nodes with small PPR values, which helps improve efficiency. In addition, {\em \ssppr+} achieves significant speedup over {\em \ssppr}, and is around 10 times faster than the latter on most of the datasets. %This is due to our advanced design of the index structure according to our theoretical analysis in Section \ref{sec:ana}.
The {\em HubPPR} also improves over {\em BiPPR}, but the improvement is far less than what {\em \ssppr+} achieves over {\em \ssppr}. %The reason is that, for single-source PPR queries, the number of required random walks is much larger than that in point-to-point PPR queries. Hence, when the stored random walks are consumed on a hub, and it needs to do random walks online.
Moreover, even without any index, {\em \ssppr} is still more efficient than {\em HubPPR}. %which indicates that the proposed {\em \ssppr} is more favorable choice on single-source PPR queries than other alternatives.

As we can observe from Table \ref{tbl:ppr-query}, with our optimization techniques introduced in Section \ref{sec:opt}, the index-free method {\em FORA} improves over {\em FORA-Basic} by up to 1.8x. Apart from the 6 public datasets, we further test the effectiveness of our methods on the four social networks from company X. We omit the results for the baseline methods (MC, BiPPR, and HubPPR) since they incur prohibitive processing costs.  As shown in Table \ref{tbl:fora-ss-opt}, {\em FORA} still improves over {\em FORA-Basic} by more than 2x almost on all datasets, which demonstrates the effectiveness of our proposed optimization technique for online algorithms. For the index-based method, {\em FORA} improves over {\em FORA+} by at least twice on almost all datasets, and up to 2.8x. As shown in Table \ref{tbl:exp-space-consumption},  the space consumption required by {\em FORA+} is twice as that of {\em FORA-Basic+}, which demonstrates that our optimization technique achieves a good trade-off between query time and space consumption.

%\begin{table}[!t]
%\centering
%\tbl{Whole-graph SSPPR performance (s). ($K=10^3$) \label{tbl:ppr-query}}{
%  \begin{tabular}{ | l | r | r|r|r |r|r|r|}
%    \hline
%        & {\em MC} & {\em BiPPR} & {\em HubPPR}&   {\em \ssppr} & {\em \ssppr-OPT} & {\em \ssppr+} & {\em \ssppr-OPT+}\\
%    \hline
% {\em DBLP}  &14.2 &	3.8&  	2.8&	0.8& 0.6	& 0.09 & 0.05  \\
%    \hline
%{\em Web-St}  & 5.4	&3.7&  	1.6	&0.03& 0.02	&  0.01& 0.01 \\
%    \hline
% {\em Pokec} &69.1	&24.9& 19.6& 11.26&	6.3 & 0.9 & 0.4 \\
%    \hline
% {\em LJ}&163.5	& 61.4& 50.8	& 15.5 & 9.9	&1.2 & 0.6 \\
%    \hline
%{\em Orkut} &230.6	& 158.2 &126.3	& 40.1& 26.4	& 4.8	& 1.7 \\
%    \hline
%{\em Twitter}   &4.3K	&3.1K& 	 2.4K & 513.8& 283.1	&63.3 &	 29.8\\
%    \hline \hline
%{\em X0}   & 2.4K	&  & 	 &  & 	&66.7 &	 \\
%    \hline
%{\em X1}   &5.3K	& & 	 &  & 	&130.7 &	 \\
%    \hline
%{\em X2}   &	& & 	 &  & 	& 152.4 &	 \\
%    \hline
%{\em X3}   &	& & 	 &  & 	&216.8 &	 \\
%    \hline
%  \end{tabular}}
%\end{table}

\begin{table}[!t]
\centering
%\tbl{Whole-graph SSPPR performance (s) (i). ($K=10^3$) \label{tbl:ppr-query}}{
\caption{Whole-graph SSPPR performance (s) (i). ($K=10^3$)}
\label{tbl:ppr-query}
  \begin{tabular}{ | l | r | r|r|r |r|r|r|}
    \hline
        & {\em MC} & {\em BiPPR} & {\em HubPPR} & {\em FORA-Basic} & {\em FORA} & {\em FORA-Basic+}&   {\em \ssppr+} \\
    \hline
 {\em DBLP}  &14.2 &	3.8&  	2.8&	0.8& 0.6	& 0.09 & 0.05 \\
    \hline
{\em Web-St}  & 5.4	&3.7&  	1.6	& 0.03& 0.02	&  0.01& 0.01 \\
    \hline
 {\em Pokec} &69.1	&24.9& 19.6& 11.26&	6.3 & 0.9 & 0.4	 \\
    \hline
 {\em LJ}&163.5	& 61.4& 50.8	& 15.5 & 9.9	&1.2 & 0.6 \\
    \hline
{\em Orkut} &230.6	& 158.2 &126.3	&  40.1& 26.4	& 4.8	& 1.7 \\
    \hline
{\em Twitter}   &4.3K	&3.1K& 	 2.4K &  513.8& 283.1	&63.3 &	 29.8\\
    \hline
  \end{tabular}%}
\end{table}




\begin{table}[!t]
\centering
%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
\caption{Whole-graph SSPPR performance (s) (ii). ($K=10^3$)}
\label{tbl:fora-ss-opt}
  \begin{tabular}{ | l | r | r|r|r|}
    \hline
        & {\em FORA-Basic} & {\em FORA} & {\em FORA-Basic+}&   {\em \ssppr+}\\
    \hline
{\em X0}   & 527.47  & 259.9	&66.7 &	31.2 \\
    \hline
{\em X1}   & 957.4 &  504.9 	&130.7 &	60.4 \\
    \hline
{\em X2}   & 1072.5 & 530.4	& 152.4 &	63.7 \\
    \hline
{\em X3}   & 2340.6 &  1163.3 	&216.8 & 97.2	 \\
    \hline
  \end{tabular}%}
\end{table}












\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{small}
    \begin{tabular}{cc}
        %\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
      	\multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\
      	
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/dblp-topk-time.eps} &
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/pokec-topk-time.eps} \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/dblp-topk-time.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/pokec-topk-time.eps} \\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\%[-1mm]

        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/orkut-topk-time.eps} &
        %\hspace{-2mm} \includegraphics[height=35mm]{./figure/new_fora/tw-topk-time.eps} \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/orkut-topk-time.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/time/tw-topk-time.eps} \\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\%[-1mm]

 \end{tabular}
 \caption{Top-$k$ SSPPR query efficiency: varying $k$.} \label{exp:topk-time}
\end{small}
\end{figure*}
\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
\begin{small}
    \begin{tabular}{cc}
        %\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
        \multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\

%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/dblp-topk-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/pokec-topk-prec.eps}\\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/dblp-topk-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/pokec-topk-prec.eps}\\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/orkut-topk-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/tw-topk-prec.eps}\\
	 	\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/orkut-topk-prec.eps} &
		\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/precision/tw-topk-prec.eps}\\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\
 \end{tabular}
 \caption{Top-$k$ SSPPR query accuracy: varying $k$.} \label{exp:topk-acc}
\end{small}
\end{figure*}

\begin{figure*}[!t]
	\centering
	%\vspace{-2mm}
	\begin{small}
		\begin{tabular}{cc}
			%\multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
			\multicolumn{2}{c}{\hspace{-8mm} \includegraphics[height=10mm]{./figure/Revision-new-figures/topk_query_legend.eps}}  \\

			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/dblp-topk-prec.eps} &
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/pokec-topk-prec.eps}\\
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/dblp-topk-ndcg.eps} &
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/pokec-topk-ndcg.eps}\\
			\hspace{-2mm} (a) DBLP  &
			\hspace{-2mm} (b) Pokec \\
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/orkut-topk-prec.eps} &
			%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/new/tw-topk-prec.eps}\\
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/orkut-topk-ndcg.eps} &
			\hspace{-2mm} \includegraphics[height=35mm]{./figure/Revision-new-figures/ndcg/tw-topk-ndcg.eps}\\
			\hspace{-2mm} (c) Orkut &
			\hspace{-2mm} (d) Twitter \\
		\end{tabular}
		\caption{Top-$k$ SSPPR query NDCG: varying $k$.} \label{exp:topk-ndcg}
	\end{small}
\end{figure*}



%\vspace{-1mm}
\subsection{Top-$\boldsymbol k$ SSPPR Queries} \label{sec:exp-topk}
%$This section evaluates the efficiency and accuracy of the proposed top-$k$ PPR query algorithms against the states-of-the-art.
%
In our second set of experiments, we evaluate the efficiency and accuracy of each method for top-$k$ SSPPR queries. For our methods, we only include our {\em FORA} and {\em FORA+} that includes the optimizations presented in Section \ref{sec:topk-running-time-guarantee} to avoid the figures being too crowded. We will examine the effectivess of our optimization techniques in the next set of experiments.


{\cblue
\subsubsection{Top-$\boldsymbol k$ query efficiency}

Figures \ref{exp:topk-time} reports the average query time of each method on four representative datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, and {\em Twitter}. (The results on the other two datasets are qualitatively similar, and are omitted due to the space constraint.) Note that the y-axis is in log-scale.
Recall that {\em Forward Push} provides no approximation guarantee, and we tune the $\rmax$ on each dataset separately, so that it provides the same precision for top-500 SSPPR queries as our {\em \ssppr} algorithm does. Similarly, for TPA \cite{yoon2018tpa}, we tune their parameters so that it provides the best possible precision.

The main observation is that our {\em \ssppr+} achieves the best performance on all the datasets. For instance, on Twitter dataset with $k=500$, our {\em \ssppr+} provides similar or better accuracy and NDCG as competitors, and runs 2x faster than TopPPR, two order of magnitude faster than MC-Topk, and more than 500x faster than Forward Push, TPA, BiPPR, and HubPPR.
This is expected since our FORA+ applies an iterative approach to refine the top-$k$ answers and terminates immediately whenever the answer could provide the desired approximation guarantee; it further uses the indexing scheme to reduce the expensive costs of random walks.

Our FORA is the fastest online algorithm except TopPPR since TopPPR uses a more advanced filter-refinement paradigm to answer the top-$k$ queries. However, their proposed approach does not benefit from indexing scheme, and is outperformed by our FORA+. It is also difficult for TopPPR to benefit from indexing scheme since {\em (i)} their random walk adopts the $\sqrt{\alpha}$-random walk, and all the nodes visited will be used to estimate the PPR scores; {\em (ii)} the sources of random walks in Monte-Carlo phase are generated randomly in TopPPR and it may results in poor cache performances. In contrast, FORA+ only need to scan the index structures in order and only stores the destinations in index structure, making it light-weighted and cache-friendly.

Another observation is that after extending the MC approach with our top-$k$ algorithm, MC-Topk achieves more than 20x speedup on Twitter over its single-source alternative. This further demonstrates the effectiveness of our top-$k$ algorithm proposed in Section \ref{sec:topk-running-time-guarantee}, which improves the time complexity to $O(\frac{\log{n}}{\epsilon^2\cdot \pi(s,v_k^*)})$. However, our FORA and FORA+ are still far more efficient than MC-Topk since FORA and FORA+ explores the forward push to reduce the random walk costs.


%Recall that {\em Forward Push} provides no approximation guarantee, and we tune the $\rmax$ on each dataset separately, so that it provides the same precision for top-500 SSPPR queries as our {\em \ssppr} algorithm does. Similarly, for TPA \cite{yoon2018tpa}, we tune their parameters so that it provides the same precision as our methods.

%Observe that, when both algorithms provide the identical precision, the performance of the proposed {\em \ssppr} and {\em Forward Push} is roughly comparable on small and medium size graphs, e.g., on {\em DBLP}, {\em Pokec}, and {\em Orkut}. When the graph size increases, however, {\em \ssppr} dominates the {\em Forward Push} in terms of the query efficiency. In particular, on {\em Twitter}, {\em \ssppr} is faster than {\em Forward Push} by two orders of magnitude. Compared with {\em TPA}, our proposed {\em \ssppr} still outperforms it by up to two order of magnitude when providing identical precision.

Finally, with our index structure, {\em \ssppr+} further improves over {\em \ssppr} by an order of magnitude, which demonstrates the effectiveness of the index structure. Notably, on the Twitter social network with 1.5 billion edges, our {\em FORA+} can answer the top-500 query in 0.8 second.

%{\em Forward Push} is practically efficient on small graphs, e.g., {\em DBLP} and {\em Pokec}, and can even outperform the proposed {\em \ssppr} on large $k$ settings, e.g., when $k=400$. However, on large graphs, the proposed {\em \ssppr} is more efficient than the Forward Push algorithm, and improves over the Forward Push algorithm by up to an order of magnitude on the Twitter dataset. Moreover, our {\em \ssppr} provides strict approximation guarantee for the top-$k$ SSPPR query, while the {\em Forward Push} provides no guarantee on the results. This indicates that our {\em \ssppr} is a preferred choice

%This indicates that our {\em \ssppr} achieves a better trade-off among the theoretical guarantee, the practical query accuracy and time efficiency than the {\em Forward Push} algorithm.



%The reason is that {\em HubPPR} requires performing a large number of backward searches, as is the case for {\em BiPPR}.
%
%%Nevertheless, even without index, our {\em \ssppr} is still several times faster than {\em HubPPR}. With full-fledged index, our {\em \ssppr+} is an order of magnitude faster than {\em HubPPR} approach.
%
\subsubsection{Top-$\boldsymbol k$ query accuracy}

To compare the accuracy of the top-$k$ results returned by each method, we first calculate the ground-truth answer of the top-$k$ queries using the {\em Power Iteration} \cite{page1999pagerank} method with 100 iterations. Afterwards, we evaluate the top-$k$ results of each algorithm by their precision and NDCG \cite{JarvelinK00} with respect to the ground truth.
Note that the precision and recall are the same for the top-$k$ SSPPR queries, and is the fraction of nodes returned by the top-$k$ algorithm that are real top-$k$ nodes.  For NDCG, let $s$ be the query node, $v_1,v_2,\cdots, v_k$ be the $k$ nodes returned by the top-$k$ algorithm, and $v_1^*, v_2^*,\cdots, v_k^*$ be the true top-$k$ nodes. Then, the NDCG is defined as $\frac{1}{Z_k}\sum_{i=1}^k{\frac{2^{\pi(s,v_i)}-1}{\log{(i+1)}}}$, where $Z_k=\sum_{i=1}^k{\frac{2^{\pi(s,v_k^*)-1}}{\log{(i+1)}}}$.


Figure~\ref{exp:topk-acc} (resp. Figure~\ref{exp:topk-ndcg}) show the accuracy (resp. NDCG) of the top-$k$ query algorithms on four datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, and {\em Twitter}. Observe that all methods except TPA consistently provide high precisions. In the meantime, notice that our FORA+ consistently provides similar precision as TopPPR and sometimes even slightly better precision than TopPPR on all the tested datasets. In terms of NDCG, all methods achieve very high NDCG scores, above 0.999 on all datasets.

%To explain, all these four algorithms include a local update algorithm, either forward push or backward push, and provides a deterministic part, i.e., $\rese(s,v)$, and then use random walks to approximate the remaining part. However, the {\em MC} approach only use the random walks to estimate the PPRs, which is less accurate than the other solutions.


\subsubsection{Scalability of Top-$\boldsymbol k$ algorithms}
In this section, we examine the scalability of our FORA+ using synthetic datasets. We first generate a synthetic dataset with the same size as Twitter and then generate a graph with 8.6 billion edges. The results are reported in Table \ref{tbl:rmat-scalability}. As we can see, our FORA+ achieves 3x improvement over TopPPR on both datasets while providing the same accuracy and NDCG. As we will see in Section \ref{sec:exp-preprocessing}, the space consumption of FORA+ is only 1.6x and 1.5x that of TopPPR on RMAT-1 and RMAT-2, respectively. This demonstrates that FORA+ achieves a better trade-off between query efficiency and space consumption when providing the same accuracy for the top-$k$ queries.
}



\subsection{Effectiveness of the Top-$\boldsymbol k$ optimization}
In this set of experiment, we evaluate the effectiveness of the new top-$k$ algorithm proposed in Section \ref{sec:topk-running-time-guarantee}, which provides improved time complexity, and reduces the time to calculate the bounds for each node. We present the results for 6 representative datasets: {\em DBLP}, {\em Pokec}, {\em Orkut}, {\em Twitter}, {\em X2}, and {\em X3}.

Figures \ref{exp:top-opt-time}(a)-(f) demonstrate the running time of {\em FORA} and {\em FORA+}, against the versions without the optimization techniques in Section \ref{sec:topk-running-time-guarantee}, referred to as {\em FORA-Basic} and {\em FORA-Basic+} for the index-free and index-based solution, respectively. As we can observe, with the new algorithm, {\em FORA} (resp. {\em FORA+} improves over {\em FORA-Basic} (resp. {\em FORA-Basic+}) by a large margin. For instance, on Twitter dataset, {\em FORA} (resp. {\em FORA+}) improves over {\em FORA-Basic} (resp. {\em FORA-Basic+}) by around 4x (resp. 6x). The main reason for the significant improvement are two-fold: (i) the time complexity of {\em FORA} and {\em FORA+} depend on $\frac{1}{\pi(s,v^*_k)}$ while {\em FORA-Basic} and {\em FORA-Basic+} depend on $\frac{1}{n}$; (ii) {\em FORA} and {\em FORA+} avoids the expensive bound calculation part that are required by {\em FORA-Basic} and {\em FORA-Basic+}.

Next, we report the accuracy of the four methods on the 6 datasets as shown in Figures \ref{exp:top-opt-acc}(a)-(f). As we can observe, all four methods provide similarly high accuracy for the top-$k$ queries on all datasets. To explain, all four methods share the similar spirit by adaptively refine the top-$k$ answer and return the approximate answer with theoretical guarantees. Therefore, all the four methods provide similarly high accuracy.



\begin{table}[!t]
	\centering
	%\tbl{Whole-graph SSPPR performance (s) (ii). ($K=10^3$) \label{tbl:fora-ss-opt}}{
	\caption{Scalability test on synthetic datasets. ($K=500$)}
	\label{tbl:rmat-scalability}
	\begin{tabular}{ | l | r | r|r|r|r|r|}
		\hline
		\multirow{2}{*}{}&  \multicolumn{2}{c|}{\bf Query Time} & \multicolumn{2}{c|}{\bf Precision} & \multicolumn{2}{c|}{\bf NDCG}\\
		\cline{2-7}
        & {RMAT-1} & {RMAT-2} & {RMAT-1} & {RMAT-2} & {RMAT-1} & {RMAT-2} \\ \hline
		{\em FORA+}   & 17.4 & 149.5	& 0.993 &	0.995 &0.9999 & 0.9999 \\
		\hline
		{\em TopPPR}   &  51.1&  481.0	& 0.993 & 0.995	 & 0.9999 & 0.9999 \\
		\hline
	\end{tabular}%}
\end{table}




\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{small}
    \begin{tabular}{cc}
          \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/topk-opt/topk-opt-algo-legend.eps}}  \\[0mm]
      %\multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figs/topk_query_legend.eps}}  \\[-2mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-dblp.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-pokec.eps} \\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\%[-1mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-orkut.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-twitter.eps} \\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\%[-1mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x2.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x3.eps} \\
        \hspace{-2mm} (e) X2 &
        \hspace{-2mm} (f) X3 \\%[-1mm]

 \end{tabular}
 \caption{Effectiveness of top-$k$ Optimization: query efficiency.} \label{exp:top-opt-time}
\end{small}
\end{figure*}

\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
\begin{small}
    \begin{tabular}{cc}
      \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/topk-opt/topk-opt-algo-legend.eps}}  \\[0mm]
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-dblp-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-pokec-prec.eps}\\
        \hspace{-2mm} (a) DBLP  &
        \hspace{-2mm} (b) Pokec \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-orkut-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-twitter-prec.eps}\\
        \hspace{-2mm} (c) Orkut &
        \hspace{-2mm} (d) Twitter \\
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x2-prec.eps} &
        \hspace{-2mm} \includegraphics[height=35mm]{./figure/topk-opt/topk-opt-x3-prec.eps}\\
        \hspace{-2mm} (e) X2 &
        \hspace{-2mm} (f) X3 \\
 \end{tabular}
 \caption{Effectiveness of top-$k$ Optimization: query accuracy.} \label{exp:top-opt-acc}
\end{small}
\end{figure*}






%\begin{figure*}[!t]
% \centering
%   %\vspace{-2mm}
%    \begin{small}
%    \begin{tabular}{cc}
%          \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
%      %\multicolumn{4}{c}{\hspace{-8mm} \includegraphics[height=2.8mm]{./figs/topk_query_legend.eps}}  \\[-2mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-dblp.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-pokec.eps} \\
%        \hspace{-2mm} (a) DBLP  &
%        \hspace{-2mm} (b) Pokec \\%[-1mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-orkut.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-twitter.eps} \\
%        \hspace{-2mm} (c) Orkut &
%        \hspace{-2mm} (d) Twitter \\%[-1mm]
%
% \end{tabular}
% \caption{Top-$k$ SSPPR query efficiency: varying $\epsilon$.} \label{exp:2topk-time}
%\end{small}
%\end{figure*}
%
%\begin{figure*}[!t]
% \centering
%   %\vspace{-2mm}
%\begin{small}
%    \begin{tabular}{cc}
%      \multicolumn{2}{c}{\hspace{-2mm} \includegraphics[height=3mm]{./figure/new/algo-legend.eps}}  \\[0mm]
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-dblp-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-pokec-prec.eps}\\
%        \hspace{-2mm} (a) DBLP  &
%        \hspace{-2mm} (b) Pokec \\
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-orkut-prec.eps} &
%        \hspace{-2mm} \includegraphics[height=35mm]{./figure/2topk/topk-epsilon-twitter-prec.eps}\\
%        \hspace{-2mm} (c) Orkut &
%        \hspace{-2mm} (d) Twitter \\
% \end{tabular}
% \caption{Top-$k$ SSPPR query accuracy: varying $\epsilon$.} \label{exp:2topk-acc}
%\end{small}
%\end{figure*}




%\vspace{-2mm}
\subsection{Preprocessing Costs}\label{sec:exp-preprocessing}


\begin{table}[!t]
\vspace{0mm}
\centering
%\hspace*{-3mm}
%\tbl{Preprocessing time.\label{tbl:exp-preprocessing-time}}{
\caption{Preprocessing time.}
\label{tbl:exp-preprocessing-time}
  \begin{tabular}{ | p{0.6in} | p{0.6in} |p{0.4in}|p{0.8in}|p{1.3in} |}
    \hline
     {\bf Datasets}  & {\em HubPPR}& {\em TPA} & {\em \ssppr+ (for whole graph)} &{\em \ssppr-Basic+} \& {\em \ssppr+ (for top-$k$)} \\
    \hline
 {\em DBLP} & 26.4& 4.4 & 7.6	& 3.6	  \\
    \hline
{\em Web-St}  &  9.3& 1.3 & 3.2 &1.5  \\
    \hline
 {\em Pokec} &90.6& 42.5 & 77.1	&34.6 \\
    \hline
 {\em LJ}& 279.9& 112.5 & 181.3	&81.2   \\
    \hline
{\em Orkut} &530.6& 177.3& 383.5 & 165.9\\
    \hline
{\em Twitter}   &5088.6& 3112.3 & 5130.4	& 2255.4	\\
    \hline\hline
    
    {\em RMAT-1} &-& -& -& 2591.2 \\
    \hline
{\em RMAT-2}   &-& - & -	& 13672.8	\\
    \hline\hline
{\em X0}   &-&- & 2031.2	&967.14	\\
\hline
{\em X1}   &-&- & 5244.5	& 2428.6	\\
\hline
{\em X2}   &-&- & 5721.7	& 2602.9	\\
\hline
{\em X3}   &-&- & 8836.4	& 4213.5	\\
\hline
  \end{tabular}%}
\end{table}

Finally, we inspect the preprocessing costs of our methods against alternatives. We first examine the preprocessing time of the index-based methods: {\em \ssppr+}, {\em \ssppr-Origin+}, {\em HubPPR}, and {\em TPA}. Note that the $\rmax$ of {\em FORA+} for whole-graph and top-$k$ queries are different, and therefore the preprocessing time are shown as seperately in Table \ref{tbl:exp-preprocessing-time}. The choice of tuned $\rmax$ of {\em FORA+} is the same as that of {\em FORA-Basic}, and therefore their preprocessing time are the same.
As shown in Table \ref{tbl:exp-preprocessing-time}, the preprocessing time of {\em \ssppr+}, {\em FORA-Basic+}, {\em HubPPR}, and {\em TPA} are all moderate. On the largest dataset {\em X3}, our {\em FORA+} for whole graph SSPPR queries (resp. for top-$k$ SSPPR queries) can still finish index construction in less than 3 hours (resp. less than 1 and half an hour), which is more than compensated by its high query performance as shown in Table \ref{tbl:ppr-query}. Besides, this preprocessing time can be further significantly reduced by parallelizing the index construction process.




\begin{table}[!t]
\vspace{0mm}
\centering
%\hspace*{-3mm}
%\tbl{Space consumption.\label{tbl:exp-space-consumption}}{
\caption{Space consumption.}
\label{tbl:exp-space-consumption}
  \begin{tabular}{|  p{0.6in}|p{0.65in}| p{0.85in} |p{0.4in}|p{0.4in}|p{1.0in}|p{0.8in} |}
    \hline
      {\bf Datasets}   & {\em MC}/{\em FORA} & {\em BiPPR/TopPPR}&{\em HubPPR} & {\em TPA} &  {\em FORA-Basic+} \& {\em FORA+} (for top-$k$) & {\em FORA+} (for whole-graph) \\
    \hline
 {\em DBLP} & 18.4MB &	36.8MB& 127.6MB	&23.3MB	& 109.2MB & 200.1MB \\
    \hline
{\em Web-St}  &  10.4MB & 20.8MB& 66.3MB  &12.6MB	& 55.9MB& 101.4MB \\
    \hline
 {\em Pokec} &130.8MB &	261.5MB & 673.5MB &143.6MB	& 542.7MB& 954.6MB\\
    \hline
 {\em LJ}& 295.2MB	&590.5MB & 1.7GB &333.6MB	&1.4GB & 2.5GB \\
    \hline
{\em Orkut} &950.1MB	&1.9GB& 3.5GB &974.9MB	& 2.6GB& 4.2GB \\
    \hline
{\em Twitter}   &6.2GB &12.5GB&  25.1GB	&6.5GB& 18.8GB & 31.4GB	\\
    \hline\hline
{\em RMAT-1}    &- &12.5GB&  -	&-& 20.0GB & -	\\\hline
{\em RMAT-2}    &- &66.5GB&  -	&-& 96.3GB & -	\\
\hline\hline
{\em X0} &  2.0GB	&-& - &-	& 7.5GB& 13.1GB \\
    \hline
{\em X1} &3.2GB	&-& - &-	& 13.2GB& 23.2GB \\
    \hline
{\em X2} &4.6GB	&-& - &-	& 17.5GB& 30.4GB \\
    \hline
{\em X3} & 6.0GB	&-& - &-	& 22.6GB& 39.2GB \\
    \hline
  \end{tabular}%}
\end{table}


Next, we examine the space consumption of all methods. Note that each method will need to store at least a copy of the graph. For {\em MC}, {\em FORA}, and {\em TPA}, they can store only a single copy of the input graph (each node stores the out-neighbor list). However, for {\em HubPPR}, {\em BiPPR} and {\em TopPPR}, they need to store two copies of the graph (each node stores an out-neighbor and an in-neighbor list) for efficient random walks and backward propagation.

Table \ref{tbl:exp-space-consumption} reports the space consumption of all methods. As we can observe, the index size of our {\em \ssppr+} for whole-graph queries and top-$k$ queries are no more than 7.5x and 4x of the original graph, respectively. The space consumption is more than compensated by the superb performance of {\em FORA+}, where we can answer a whole-graph query within 30 seconds and  top-$k$ query within 0.9 second on the 1.5 billion edge Twitter graph, which improves over the index-free {\em FORA} by more than an order of magnitude on almost all datasets. This demonstrates the effectiveness and efficiency of our indexing scheme. 
{\cblue

Compared to TopPPR, FORA+ achieves 2x, 3x, and 3.4x improvement on Twitter, RMAT-1, and RMAT-2, with only 1.5x, 1.6x, and 1.5 space consumption, respectively. 
%Besides, even without index, our {\em FORA} can still outperform all alternative index-free and index-based methods on whole-graph SSPPR queries and  top-$k$ SSPPR queries by a large margin. 
The experimental results demonstrate that our proposed methods achieve a good trade-off between the space consumption and query efficiency when providing query answers with identical accuracy.
}


\begin{figure*}[!t]
 \centering
   %\vspace{-2mm}
    \begin{tabular}{cc}
    \hspace{-4mm} \includegraphics[height=2.4mm]{./figure/topk-tune-rmax/tune-rmax-legend1.eps} & \hspace{8mm}\includegraphics[height=2.4mm]{./figure/topk-tune-rmax/tune-rmax-legend2.eps} \\[0mm]
        \hspace{-4mm}  \includegraphics[height=35mm]{./figure/topk-tune-rmax/rmax-vs-query1.eps} &
         \hspace{8mm} \includegraphics[height=35mm]{./figure/topk-tune-rmax/rmax-vs-query2.eps}\\
        \hspace{-4mm} (a)   &
        \hspace{8mm}(b)  \\

 \end{tabular}
 \caption{Tunning $\rmax$ for top-$k$ SSPPR queries ($\times\rmax^*$)}. \label{exp:top-tune-rmax}
\end{figure*}





Finally, we examine the trade-off between the space consumption and top-$k$ query performance of our {\em FORA+} algorithm by tuning $\rmax$.  Let $\rmax^*$ be the $\rmax$ value set according to Section \ref{sec:ana}. We then set $\rmax$ to $\rmax^*$, $3\rmax^*$, $5\rmax^*$, and $7\rmax^*$. Notice that, the index size is proportional to $\rmax$ and let $y$ be the index size when $\rmax = \rmax^*$. Then, the index size will be $y$, $3y$, $5y$, and $7y$, respectively. As we can observe, when we increase the index size for {\em FORA+}, the query performance also improves on almost all datasets. To explain, by increasing the index size, {\em FORA+} avoids the expensive random walks and thus saving the query time. However, from the experiment, we can observe that when $\rmax = \rmax^*$, it actually achieves the best trade-off between the query performance and space consumption, and hence in our experiment, we set $\rmax=\rmax^*$ for all the top-$k$ queries.

